Controlled-Phase Gate by Dynamic Coupling of Photons to a Two-Level Emitter

We propose an architecture for achieving high-fidelity deterministic quantum logic gates on dual-rail encoded photonic qubits by letting photons interact with a two-level emitter (TLE) inside an optical cavity. The photon wave packets that define the qubit are preserved after the interaction due to a quantum control process that actively loads and unloads the photons from the cavity and dynamically alters their effective coupling to the TLE. The controls rely on nonlinear wave mixing between cavity modes enhanced by strong externally modulated electromagnetic fields or on AC Stark shifts of the TLE transition energy. We numerically investigate the effect of imperfections in terms of loss and dephasing of the TLE as well as control field miscalibration. Our results suggest that III-V quantum dots in GaAs membranes is a promising platform for photonic quantum information processing.

==> app_numerical_implementation.tex <==
% ----------------------------------------------------------------
\section{Numerical Solution of Equations of Motion}
% ----------------------------------------------------------------

% ----------------------------------------------------------------
\subsection{Control Field $\Omega(t)$}
% ----------------------------------------------------------------

In section~\secref{gate performance}, the \texttt{Julia} package \texttt{SmoothingSplines} was used to generate the control field $\Omega(t)$ by interpolating between a discrete set of values, $\Omega_n\!\equiv\! \Omega(t_n)$, with $n\!\in\![1,N_{\Omega}]$. We limited the bandwidth of $\Omega(t)$ by keeping a fixed characteristic "smoothing" time, $\tau_{\rm{spline}}$, required by the \texttt{SmoothingSplines} algorithm.
% 
% \begin{align}
%     \ket{\phi} = 
% \end{align} 








% % 
% and the state of the photon (after the first beam splitter) is
% % 
% \begin{align}
%     \ket{\psi} = \frac{1}{\sqrt{2}}\Big(\ket{u} + \ket{d}\Big).
% \end{align} 
% %
% The effect of the scattering is 
% % 
% \begin{multline}
%   \frac{1}{2\sqrt{2}}  \Big( \ket{\uparrow}_A + e^{i\phi_A}\ket{\downarrow}_A \Big) \otimes \Big( \ket{\uparrow}_B + e^{i\phi_B}\ket{\downarrow}_B \Big) \otimes \Big(\ket{u} + \ket{d}\Big) \rightarrow \\
%   \frac{1}{2\sqrt{2}}  \Big( t_A \ket{\uparrow}_A + e^{i\phi_A}\ket{\downarrow}_A \Big) \otimes \Big( \ket{\uparrow}_B + e^{i\phi_B}\ket{\downarrow}_B \Big)\otimes  \ket{u} + \frac{1}{2\sqrt{2}}  \Big( \ket{\uparrow}_A + e^{i\phi_A}\ket{\downarrow}_A \Big) \otimes \Big( t_B \ket{\uparrow}_B + e^{i\phi_B}\ket{\downarrow}_B \Big)\otimes  \ket{d}.
% \end{multline} 
% %
% This is the modified version of Eq. (4.10). According to Eq. (4.11), the second beam splitter causes the transformation
% % 
% \begin{align}
%     \ket{u} \rightarrow \frac{1}{\sqrt{2}} \Big( \ket{u} - \ket{d} \Big) , ~\text{and} ~ \ket{d} \rightarrow \frac{1}{\sqrt{2}} \Big( \ket{u} + \ket{d} \Big).
% \end{align} 
% %
% The state is then
% % 
% \begin{multline}
%   \ket{\Psi} = \frac14 \Big( t_A \ket{\uparrow}_A + e^{i\phi_A}\ket{\downarrow}_A \Big) \otimes \Big( \ket{\uparrow}_B + e^{i\phi_B}\ket{\downarrow}_B \Big)\otimes  \Big( \ket{u} - \ket{d} \Big) ~+\\
%   \frac14  \Big( \ket{\uparrow}_A + e^{i\phi_A}\ket{\downarrow}_A \Big) \otimes \Big( t_B \ket{\uparrow}_B + e^{i\phi_B}\ket{\downarrow}_B \Big)\otimes  \Big( \ket{u} + \ket{d} \Big) = \\
%   \frac14 \Big[ \big(t_A + t_B)\ket{\uparrow\uparrow} + e^{i\phi_A}\big(1+t_B\big)\ket{\downarrow\uparrow} +  e^{i\phi_B}\big(1+t_A\big)\ket{\uparrow\downarrow} + 2 e^{i(\phi_A+\phi_B)} \ket{\downarrow\downarrow} \Big] \ket{u} ~+ \\ 
%   \frac14 \Big[ \big(t_B - t_A)\ket{\uparrow\uparrow} + e^{i\phi_A}\big(t_B-1\big)\ket{\downarrow\uparrow} +  e^{i\phi_B}\big(1-t_A\big)\ket{\uparrow\downarrow}  \Big] \ket{d}
% \end{multline} 
% %

% % The state is then
% % % 
% % \begin{multline}
% %   \ket{\Psi} = \frac14 \Big( t_A e^{i\phi_A}\ket{\uparrow}_A + \ket{\downarrow}_A \Big) \otimes \Big( e^{i\phi_B}\ket{ \uparrow}_B + \ket{\downarrow}_B \Big)\otimes  \Big( \ket{u} - \ket{d} \Big) ~+\\
% %   \frac14  \Big( e^{i\phi_A} \ket{ \uparrow}_A + \ket{\downarrow}_A \Big) \otimes \Big( t_B e^{i\phi_B}\ket{\uparrow}_B + \ket{\downarrow}_B \Big)\otimes  \Big( \ket{u} + \ket{d} \Big) = \\
% %   \frac14 \Big[ \big(t_A + t_B)e^{i(\phi_A+\phi_B)}\ket{\uparrow\uparrow} + e^{i\phi_A}\big(1+t_B\big)\ket{\downarrow\uparrow} +  e^{i\phi_B}\big(1+t_A\big)\ket{\uparrow\downarrow} + 2 e^{i(\phi_A+\phi_B)} \ket{\downarrow\downarrow} \Big] \ket{u} ~+ \\ 
% %   \frac14 \Big[ \big(t_B - t_A)\ket{\uparrow\uparrow} + e^{i\phi_A}\big(t_B-1\big)\ket{\downarrow\uparrow} +  e^{i\phi_B}\big(1-t_A\big)\ket{\uparrow\downarrow}  \Big] \ket{d}
% % \end{multline} 
% % %

% % The state after the qubits but before the second beam splitter is [compare here to Eq. (4.10)]
% % % 
% % \begin{align}
% %     \ket{\Psi} = \frac{1}{2\sqrt{2}} \Big( t_A\ket{\uparrow}_A + e^{i\phi_A}\ket{\downarrow}_A \Big) \otimes \Big( t_B\ket{\uparrow}_B + e^{i\phi_B}\ket{\downarrow}_B \Big) \otimes \Big(\ket{u} + \ket{d}\Big)
% % \end{align} 
% % %

% % Now we follow the calculation from Eq. (4.10) with this new initial state
% % % 
% % \begin{subequations}\eqlab{4.10}
% % \begin{align}
% %     \ket{\Psi} = \frac{1}{2\sqrt{2}}\Big( \ket{\uparrow}_A + e^{i\phi_A}\ket{\downarrow}_A \Big) \otimes \Big( \ket{\uparrow}_B + e^{i\phi_B}\ket{\downarrow}_B \Big) \otimes \Big(\hat{u}^\dagger + \hat{d}^\dagger \Big)\ket{\emptyset}
% %     % 14 \Big( t_1^2\ket{\uparrow} + e^{i\phi_1}\ket{\downarrow} \Big) \otimes \Big( \ket{\uparrow} + e^{i\phi_2}\ket{\downarrow} \Big) \otimes (\hat{u}^\dagger)^2 \ket{\emptyset}
% % \end{align} 
% % \end{subequations}
% % %


==> texdef.tex <==
% %%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %               Newcommand%%%%%%%%%%%%%%%%


 %LABELS
\newcommand{\eqlab}[1]{\label{eq:#1}}
\renewcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\eqsref}[2]{Eqs.~(\ref{eq:#1}) and~(\ref{eq:#2})}
\newcommand{\eqsrefplural}[2]{Eqs.~(\ref{eq:#1})-(\ref{eq:#2})}
\newcommand{\exref}[1]{\ref{ex:#1}}
\newcommand{\exlab}[1]{\label{ex:#1}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figsref}[2]{Figs.~\ref{fig:#1} and~\ref{fig:#2}}
\newcommand{\figlab}[1]{\label{fig:#1}}
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\chapsref}[2]{Chapters~\ref{chap:#1} and~\ref{chap:#2}}
\newcommand{\chaplab}[1]{\label{chap:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\secsref}[2]{Sections~\ref{sec:#1} and~\ref{sec:#2}}
\newcommand{\seclab}[1]{\label{sec:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\tabsref}[2]{Tables~\ref{tab:#1} and~\ref{tab:#2}}
\newcommand{\tablab}[1]{\label{tab:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\appsref}[2]{Appendices~\ref{app:#1} and~\ref{app:#2}}
\newcommand{\applab}[1]{\label{app:#1}}

\newcommand{\equal}{\!=\!}
\newcommand{\minus}{\!-\!}
\newcommand{\plus}{\!+\!}

\newcommand{\ket}[1]{|{#1}\rangle}
\newcommand{\bra}[1]{\langle {#1}|}
\newcommand{\expect}[1]{\big \langle {#1} \big \rangle}
\newcommand{\braket}[2]{\langle #1 | #2 \rangle}
\newcommand{\bigbra}[1]{\big\langle #1 \big|}
\newcommand{\bigket}[1]{\big| #1 \big\rangle}
\newcommand{\bigbraket}[2]{\big\langle #1 \big| #2 \big\rangle}

\newcommand{\nn}{\nonumber}
\newcommand{\gamsub}[1]{\gamma_{ #1 }}
% \newcommand{\tauin}{\tau_{ \rm{in}}}
\newcommand{\tauG}{\tau_{\!\scriptscriptstyle \mathcal{G}}}
\newcommand{\OmG}{\Omega_{\scriptscriptstyle \mathcal{G}}}
\newcommand{\tauO}{\tau_{\rm{o}}}
\newcommand{\tauI}{\tau_{\rm{i}}}
\newcommand{\tauenv}{\tau_{ \rm{e}}}
\newcommand{\Tin}{T_{\rm{in}}}
\newcommand{\Tout}{T_{\rm{out}}}
% \newcommand{\Tstore}{T_{\rm{st}}}
\newcommand{\Tstore}{T_{}}
\newcommand{\chill}{\chi^{\scriptscriptstyle (2)} }
\newcommand{\chilll}{\chi^{\scriptscriptstyle (3)} }

\newcommand{\ms}[1]{\mbox{\scriptsize #1}}
\newcommand{\msb}[1]{\mbox{\scriptsize $\mathbf{#1}$}}
\newcommand{\msi}[1]{\mbox{\scriptsize\textit{#1}}}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newcommand{\vsubsup}[3]{\bm{#1}_{#2}^{\scriptscriptstyle #3}}
% \newcommand{\ssubsup}[3]{{#1}_{#2}^{\scriptscriptstyle #3}}
% \newcommand{\ssup}[2]{{#1}^{\scriptscriptstyle #2}}
% \newcommand{\vsup}[2]{\bm{#1}^{\scriptscriptstyle #2}}
% \newcommand{\ssub}[2]{{#1}_{#2}}
% \newcommand{\vsub}[2]{\bm{#1}_{#2}}
% \newcommand{\omSub}[1]{\omega_{ #1 }}
% \newcommand{\lamSub}[1]{\lambda_{ #1 }}
% \newcommand{\delSub}[1]{\delta_{ #1 }}
% \newcommand{\tauSub}[1]{\tau_{ #1 }}
% \newcommand{\tausub}[1]{\tau_{\scriptscriptstyle #1 }}
% \newcommand{\GamSub}[1]{\Gamma_{ #1 }}
% \newcommand{\lamFSR}{\lambda_{\scriptscriptstyle \text{FSR}}}
% \newcommand{\OmFSR}{\Omega_{\scriptscriptstyle \text{FSR}}}
% \newcommand{\omout}{\omega_{ \text{out}}}
% \newcommand{\hatdsub}[2]{\hat{#1}^{\dagger}_{ #2}}
% \newcommand{\hatsub}[2]{\hat{#1}_{#2}}
% \newcommand{\so}[1]{s_{\rm{out}, #1}}
% \newcommand{\si}[1]{s_{\rm{in}, #1}}
% \newcommand{\So}[1]{S_{\rm{out}, #1}}
% \newcommand{\Si}[1]{S_{\rm{in}, #1}}
% \newcommand{\hatso}[1]{\hat{s}_{\rm{out}, #1}}
% \newcommand{\hatsi}[1]{\hat{s}_{\rm{in}, #1}}
% \newcommand{\omref}{\omega_{\text{ref} }}

% \newcommand{\subs}[2]{{#1}_{\scriptscriptstyle #2}}
% \newcommand{\dotsub}[2]{\dot{#1}_{\scriptscriptstyle #2}}
% \newcommand{\Usub}[1]{U_{\scriptscriptstyle #1}}
% % \newcommand{\hatdsub}[2]{\hat{#1}^{\dagger}_{\scriptscriptstyle #2}}
% % \newcommand{\hatsub}[2]{\hat{#1}_{\scriptscriptstyle #2}}
% \newcommand{\hbsub}[1]{\hat{b}_{\scriptscriptstyle #1}}
% \newcommand{\hasub}[1]{\hat{a}_{\scriptscriptstyle #1}}
% % \newcommand{\GamSub}[1]{\Gamma_{ #1}}
% \newcommand{\Gamsub}[1]{\Gamma_{\scriptscriptstyle #1}}
% % \newcommand{\gamsub}[1]{\gamma_{\scriptscriptstyle #1}}
% \newcommand{\chisub}[1]{\chi_{\scriptscriptstyle #1}}
% \newcommand{\Ksub}[1]{K_{\scriptscriptstyle #1}}
% \newcommand{\fsub}[1]{f_{\scriptscriptstyle #1}}
% \newcommand{\Tsub}[1]{T_{\scriptscriptstyle #1}}
% \newcommand{\PhiFP}{\Phi_{\scriptscriptstyle \text{FP}}}
% \newcommand{\Psub}[1]{P_{\scriptscriptstyle #1}}
% \newcommand{\tzeta}{\tilde{\zeta}}
% \newcommand{\DelomFWHM}{\Delta\omega_{\scriptscriptstyle \text{FWHM}}}
% \newcommand{\omFSR}{\Delta\omega_{\scriptscriptstyle \text{FSR}}}
% % \newcommand{\lamFSR}{\Delta\lambda_{\scriptscriptstyle \text{FSR}}}
% \newcommand{\tLorentz}{t_{\scriptscriptstyle \text{Lor}}}
% \newcommand{\tauRT}{\tau_{\scriptscriptstyle \text{RT}}}
% \newcommand{\tauL}{\tau_{\scriptscriptstyle L}}
% \newcommand{\lamres}{\lambda_{\text{res}}}
% \newcommand{\omres}{\omega_{\text{res}}}
% \newcommand{\LRT}{L_{\scriptscriptstyle \text{RT}}}


% \newcommand{\alphawg}{\alpha_{\text{wg}}}
% \newcommand{\alphaloss}{\alpha_{\text{loss}}}
% \newcommand{\vMsub}[1]{\boldsymbol{M}_{\scriptscriptstyle #1}}
% \newcommand{\thetasub}[1]{\theta_{\scriptscriptstyle #1}}
% \newcommand{\dotasub}[1]{\dot{a}_{\scriptscriptstyle #1}}
% \newcommand{\dotbsub}[1]{\dot{b}_{\scriptscriptstyle #1}}
% \newcommand{\dotfsub}[1]{\dot{f}_{\scriptscriptstyle #1}}
% \newcommand{\dotusub}[1]{\dot{u}_{\scriptscriptstyle #1}}
% \newcommand{\dotlamsub}[1]{\dot{\lambda}_{\scriptscriptstyle #1}}
% \newcommand{\asub}[1]{a_{\scriptscriptstyle #1}}
% \newcommand{\bsub}[1]{b_{\scriptscriptstyle #1}}
% % \newcommand{\ssub}[1]{s_{\scriptscriptstyle #1}}
% \newcommand{\Ssub}[1]{S_{\scriptscriptstyle #1}}
% \newcommand{\rsub}[1]{r_{\scriptscriptstyle #1}}
% \newcommand{\tsub}[1]{t_{\scriptscriptstyle #1}}
% \newcommand{\usub}[1]{u_{\scriptscriptstyle #1}}
% % \newcommand{\vsub}[1]{v_{\scriptscriptstyle #1}}
% \newcommand{\vvsub}[1]{\boldsymbol{v}_{\scriptscriptstyle #1}}
% \newcommand{\dsub}[1]{d_{\scriptscriptstyle #1}}
% \newcommand{\stildesub}[1]{\tilde{s}_{\scriptscriptstyle #1}}
% \newcommand{\delsub}[1]{\delta_{\scriptscriptstyle #1}}
% \newcommand{\epssub}[1]{\epsilon_{\scriptscriptstyle #1}}
% \newcommand{\Delsub}[1]{\Delta_{\scriptscriptstyle #1}}
% \newcommand{\gamsub}[1]{\gamma_{\scriptscriptstyle #1}}
% \newcommand{\omsub}[1]{\omega_{\scriptscriptstyle #1}}
% \newcommand{\lamsub}[1]{\lambda_{\scriptscriptstyle #1}}
% %\newcommand{\thetasub}[1]{\theta_{\scriptscriptstyle #1}}
% \newcommand{\phisub}[1]{\phi_{\scriptscriptstyle #1}}
% \newcommand{\phieff}{\phi_{\text{eff}}}
% %\newcommand{\phing}{\phi_{\text{eff}}}
% \newcommand{\Telec}{\tau_{\text{e}}}
% \newcommand{\Tasd}{t_{\text{asd}}}
% \newcommand{\tauc}{\tau_{\scriptscriptstyle Nc}}
% \newcommand{\tc}{t_{\scriptscriptstyle Nc}}
% \newcommand{\tf}{t_{\scriptscriptstyle Nf}}
% \newcommand{\tauNf}{\tau_{\scriptscriptstyle Nf}}
% \newcommand{\tauPon}{\tau_{\scriptscriptstyle Pon}}
% %\newcommand{\taupPoff}{\tau'_{\scriptscriptstyle \text{off}}}
% %\newcommand{\tauSoff}{\tau_{\scriptscriptstyle Soff}}
% \newcommand{\Ntraj}{N_{\text{traj}}}
% \newcommand{\Tbin}{\tau_{\text{bin}}}
% %\newcommand{\Tcollapse}{t_{\text{col}}}
% \newcommand{\Trel}{t_{\text{rel}}}
% \newcommand{\Tjit}{\tau_{\text{jit}}}
% %\newcommand{\TPoff}{T_{\scriptscriptstyle Poff}}
% %\newcommand{\TPon}{T_{\scriptscriptstyle Pon}}

% \newcommand{\mytimes}{\!\times\!}
% %\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
% %\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
% %\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
% %\newcommand{\figlab}[1]{\label{fig:#1}}
% %\newcommand{\eqlab}[1]{\label{eq:#1}}
% %\newcommand{\eqreff}[1]{Eq.~(\ref{eq:#1})}
% %\newcommand{\eqsreff}[2]{Eqs.~(\ref{eq:#1}) and~(\ref{eq:#2})}
% \newcommand{\ic}{\text{i}}
% \newcommand{\nn}{\nonumber}
% \newcommand{\gamW}{\gamma_{\scriptscriptstyle W}}
% \newcommand{\tRTN}{t_{\scriptscriptstyle RTn}}
% \newcommand{\psiOFF}{\psi_{\scriptscriptstyle off}}
% \newcommand{\psiON}{\psi_{\scriptscriptstyle on}}
% %\newcommand{\QWon}{Q_{\scriptscriptstyle Won}}
% %\newcommand{\gamWon}{\gamma_{\scriptscriptstyle Won}}
% %\newcommand{\phiRT}{\phi_{\text{\tiny{RT}}}}
% %\newcommand{\Lphi}{L_{\phi}}
% %\newcommand{\Leff}{L_{eff}}
% \newcommand{\om}{\omega}
% \newcommand{\nefft}{\tilde{n}_{\text{eff}}}
% %\newcommand{\neff}{n_{\text{eff}}}
% %\newcommand{\omref}{\omega_{\text{ref}}}
% %\newcommand{\MOmt}{\tilde{\mathbf{\Omega}}}
% %\newcommand{\MGam}{\mathbf{\Gamma}}
% %\newcommand{\delGP}{\delta_{gp}}
% \newcommand{\delGN}{\delta_{gn}}
% %\newcommand{\delP}{\delta_{p}}
% %\newcommand{\vsin}{\mathbf{s}_{+}}
% %\newcommand{\vsout}{\mathbf{s}_{-}}
% %\newcommand{\MKap}{\mathbf{K}}
% %\newcommand{\MVinv}{\mathbf{V^{\text{\tiny{-1}}}}}
% %\newcommand{\MV}{\mathbf{V}}
% %\newcommand{\gGP}{g_{gp}}
% %\newcommand{\gamP}{\gamma_{p}}
% %\newcommand{\gamGP}{\gamma_{gp}}
% \newcommand{\gN}{g_{n}}
% %\newcommand{\gGS}{g_{gs}}
% \newcommand{\gamN}{\gamma_{n}}
% %\newcommand{\gamS}{\gamma_{s}}
% \newcommand{\gamGN}{\gamma_{gn}}
% %\newcommand{\gGI}{g_{gi}}
% %\newcommand{\gamI}{\gamma_{i}}
% %\newcommand{\gamGI}{\gamma_{gi}}
% %\newcommand{\gamGS}{\gamma_{gs}}
% %\newcommand{\gamWP}{\gamma_{\scriptscriptstyle Wp}}
% \newcommand{\gamWN}{\gamma_{\scriptscriptstyle Wn}}
% %\newcommand{\va}{\mathbf{a}}
% %\newcommand{\dotaP}{\dot{a}_{p}}
% %\newcommand{\dotaGP}{\dot{a}_{gp}}
% \newcommand{\omGPt}{\tilde{\omega}_{gp}}
% %\newcommand{\omPt}{\tilde{\omega}_{p}}
% \newcommand{\omGNt}{\tilde{\omega}_{gn}}
% \newcommand{\omGN}{\omega_{gn}}
% \newcommand{\omNt}{\tilde{\omega}_{n}}
% %\newcommand{\omtP}{\tilde{\omega}_{p}}
% %\newcommand{\omtS}{\tilde{\omega}_{s}}
% %\newcommand{\omtI}{\tilde{\omega}_{i}}
% \newcommand{\Lambdat}{\tilde{\Lambda}}
% \newcommand{\LambdatNM}{\tilde{\Lambda}_{nm}}
% \newcommand{\LambdatSM}{\tilde{\Lambda}_{sm}}
% \newcommand{\omPtm}{\overline{\tilde{\omega}}_{p}}
% %\newcommand{\delN}{\delta_{n}}
% \newcommand{\DelI}{\Delta_{i}}
% \newcommand{\DelS}{\Delta_{s}}
% \newcommand{\DeliM}{\Delta_{im}}
% \newcommand{\DeliK}{\Delta_{ik}}
% \newcommand{\DelsL}{\Delta_{sl}}
% %\newcommand{\DelSl}{\Delta_{s1}}
% \newcommand{\DelsM}{\Delta_{sm}}
% \newcommand{\DelnM}{\Delta_{nm}}
% \newcommand{\omN}{\omega_{n}}
% %\newcommand{\omS}{\omega_{s}}
% %\newcommand{\omGS}{\omega_{gs}}
% \newcommand{\omtN}{\tilde{\omega}_{n}}
% \newcommand{\gamLN}{\gamma_{\scriptscriptstyle Ln}}
% %\newcommand{\MLam}{\tilde{\mathbf{\Lambda}}}
% %\newcommand{\vyout}{\mathbf{y}_{\text{out}}}
% %\newcommand{\vyin}{\mathbf{y}_{\text{in}}}
% %\newcommand{\vx}{\mathbf{x}}
% %\newcommand{\vy}{\mathbf{y}}
% %\newcommand{\vs}{\mathbf{s}}
% %\newcommand{\IM}[1]{\mbox{Im}\left\{#1\right\}}
% %\newcommand{\RE}[1]{\mbox{Re}\left\{#1\right\}}
% %\newcommand{\kapSM}{\kappa_{sm}}
% %\newcommand{\kapWN}{\kappa_{\scriptscriptstyle Wn}}
% %\newcommand{\kapLN}{\kappa_{\scriptscriptstyle Ln}}
% %\newcommand{\kapWM}{\kappa_{\scriptscriptstyle Wm}}
% %\newcommand{\kapLM}{\kappa_{\scriptscriptstyle Lm}}
% %\newcommand{\kapLNM}{\kappa_{\scriptscriptstyle Lnm}}
% %\newcommand{\kapWNM}{\kappa_{\scriptscriptstyle Wnm}}
% %\newcommand{\kapWSl}{\kappa_{\scriptscriptstyle Ws1}}
% %\newcommand{\kapWI}{\kappa_{\scriptscriptstyle Wi}}
% %\newcommand{\kapLI}{\kappa_{\scriptscriptstyle Li}}
% %\newcommand{\kapLSl}{\kappa_{\scriptscriptstyle Ls1}}
% \newcommand{\chieff}{\chi_{\text{eff}}^{(3)}}
% \newcommand{\chiM}{\chi_{m}}
% \newcommand{\xhat}{\hat{x}}
% \newcommand{\ahat}{\hat{a}}
% %\newcommand{\CLN}{\hat{C}_{\scriptscriptstyle Ln}}
% %\newcommand{\CWN}{\hat{C}_{\scriptscriptstyle Wn}}
% \newcommand{\Qintr}{Q_{\scriptscriptstyle L}}
% \newcommand{\QW}{Q_{\scriptscriptstyle W}}
% \newcommand{\tauintr}{\tau_{intr}}
% \newcommand{\Delt}{\Delta{}t}
% \newcommand{\Deltau}{\Delta{}\tau}
% \newcommand{\DelT}{\tau_{\scriptscriptstyle D}}
% \newcommand{\nave}{\langle n \rangle}
% \newcommand{\uk}{u_k}
% \newcommand{\ukq}{u_{kq}}
% \newcommand{\uki}{u_{ki}}
% \newcommand{\ukf}{u_{kf}}
% \newcommand{\uq}{u_q}
% \newcommand{\Vkq}{V_{q}}
% \newcommand{\Vnotkq}{V_{\overline{q}}}
% \newcommand{\UWq}{U_{\scriptscriptstyle Wq}}
% \newcommand{\UWl}{U_{\scriptscriptstyle Wl}}
% \newcommand{\UWLq}{U_{\scriptscriptstyle WLq}}
% \newcommand{\UWnotLq}{U_{\scriptscriptstyle Wq\overline{L}}}
% \newcommand{\UWnotLk}{U_{\scriptscriptstyle Wk\overline{L}}}
% \newcommand{\UnotWq}{U_{\scriptscriptstyle \overline{Wq}}}
% \newcommand{\Uq}{U_q}
% \newcommand{\DelN}{\Delta{}N}
% \newcommand{\tNq}{t_{N_q}}
% \newcommand{\Pmulti}{P_{\text{multi}}}
% \newcommand{\Ploss}{P_{\text{loss}}}
% \newcommand{\notD}{\overline{D}}
% \newcommand{\Pow}{\mathcal{P}}
% \newcommand{\PowNk}{\mathcal{P}_{\scriptscriptstyle Nk}}
% \newcommand{\Psum}{P_{_{\sum}}}
% \newcommand{\tqM}{t_{0q}}
% \newcommand{\tfM}{t_{0f}}
% \newcommand{\tqP}{t_q^{+}}
% %\newcommand{\tq}{t_q}
% \newcommand{\tk}{t_k}
% \newcommand{\GamDC}{\Gamma_{\text{\tiny{DC}}}}
% \newcommand{\notL}{\overline{L}}
% \newcommand{\tj}{t_j}
% \newcommand{\LqM}{L_q^{-}}
% \newcommand{\LqP}{L_q^{+}}
% \newcommand{\notLqP}{\overline{L_q^{+}}}
% \newcommand{\notLqM}{\overline{L_q^{-}}}
% \newcommand{\uNq}{u_{\scriptscriptstyle Nq}}
% \newcommand{\UNq}{U_{\scriptscriptstyle Nq}}
% \newcommand{\fNq}{f_{\scriptscriptstyle Nq}}
% \newcommand{\uNk}{u_{\scriptscriptstyle Nk}}
% \newcommand{\uNf}{u_{\scriptscriptstyle Nf}}
% \newcommand{\UNk}{U_{\scriptscriptstyle Nk}}
% \newcommand{\fNk}{f_{\scriptscriptstyle Nk}}
% \newcommand{\tNk}{t_{\scriptscriptstyle Nk}}
% \newcommand{\tauNk}{\tau_{\scriptscriptstyle Nk}}
% \newcommand{\Tdelay}{\Delta T}
% \newcommand{\DqM}{D_{0q}}
% \newcommand{\DfM}{D_{0f}}
% \newcommand{\DqP}{D_{q}^{+}}
% \newcommand{\Dq}{D_{q}}
% \newcommand{\Dlq}{D_{\scriptscriptstyle \mathcal{F}q}}
% \newcommand{\DlNO}{D_{\scriptscriptstyle \mathcal{FO}}}
% \newcommand{\Dlk}{M_{k}}
% \newcommand{\Dlj}{M_{j}}
% \newcommand{\mcDlk}{\mathcal{M}_{k}}
% \newcommand{\mcDkq}{\mathcal{M}_{q}}
% \newcommand{\DlM}{D_{0l}}
% \newcommand{\Dk}{D_{k}}
% \newcommand{\Dl}{D_{l}}
% \newcommand{\notDqM}{\overline{D_{0q}}}
% \newcommand{\notDkM}{\overline{D_{0k}}}
% \newcommand{\notDfM}{\overline{D_{0f}}}
% \newcommand{\notDkq}{\overline{D_{kq}}}
% \newcommand{\notDkc}{\overline{D_{kc}}}
% \newcommand{\tcM}{t_{0c}}
% \newcommand{\DcM}{D_{0c}}
% \newcommand{\notDcM}{\overline{D_{0c}}}
% \newcommand{\fNf}{f_{\scriptscriptstyle Nf}}
% \newcommand{\UNf}{U_{\scriptscriptstyle Nf}}
% \newcommand{\UNc}{U_{\scriptscriptstyle Nc}}
% \newcommand{\DNf}{D_{\scriptscriptstyle Nf}}
% \newcommand{\notDq}{\overline{D_{q}}}
% \newcommand{\notDk}{\overline{D_{k}}}
% \newcommand{\notMcDqM}{\overline{\mathcal{D}_{0q}}}
% \newcommand{\notMcDkM}{\overline{\mathcal{D}_{0k}}}
% \newcommand{\DkM}{D_{0k}}
% \newcommand{\Dkq}{D_{kq}}
% \newcommand{\Dkc}{D_{0c}}
% \newcommand{\Lkc}{L_{kc}}
% \newcommand{\Lqc}{L_{qc}}
% \newcommand{\Ljq}{L_{jq}}
% \newcommand{\Ljc}{L_{jc}}
% \newcommand{\Llq}{L_{lq}}
% \newcommand{\Lkq}{L_{kq}}
% \newcommand{\Wkq}{W_{kq}}
% \newcommand{\Wjq}{W_{jq}}
% \newcommand{\Ijq}{\mathcal{I}_{jq}}
% %\newcommand{\Il}{\mathcal{I}_{l}}
% \newcommand{\Ijl}{\mathcal{I}_{jl}}
% \newcommand{\jWk}{{}_jW_k}
% \newcommand{\jWl}{{}_jW_l}
% \newcommand{\kWl}{{}_kW_l}
% \newcommand{\qWk}{{}_qW_k}
% \newcommand{\lWk}{{}_lW_k}
% \newcommand{\kWq}{{}_kW_q}
% \newcommand{\lWq}{{}_lW_q}
% \newcommand{\notIkq}{\overline{\mathcal{I}_{kq}}}
% \newcommand{\notIjq}{\overline{\mathcal{I}_{jq}}}
% \newcommand{\notWkq}{\overline{W_{kq}}}
% \newcommand{\notWjq}{\overline{W_{jq}}}
% \newcommand{\notWlq}{\overline{W_{lq}}}
% \newcommand{\notjWl}{\overline{{}_jW_l}}
% \newcommand{\notjWk}{\overline{{}_jW_k}}
% \newcommand{\notlWq}{\overline{{}_lW_q}}
% \newcommand{\notlWk}{\overline{{}_lW_k}}
% \newcommand{\notLkc}{\overline{L_{kc}}}
% \newcommand{\notLOc}{\overline{L_{0c}}}
% \newcommand{\notLqc}{\overline{L_{qc}}}
% \newcommand{\notLkq}{\overline{L_{kq}}}
% \newcommand{\notLjq}{\overline{L_{jq}}}
% \newcommand{\notLjc}{\overline{L_{jc}}}
% \newcommand{\tqk}{t_{qk}}
% \newcommand{\tkc}{t_{kc}}
% \newcommand{\tqc}{t_{qc}}
% \newcommand{\tkq}{t_{kq}}
% \newcommand{\tkM}{t_{0k}}
% \newcommand{\tokc}{t_{\overline{k}c}}
% \newcommand{\tokq}{t_{\overline{k}q}}
% \newcommand{\tojq}{t_{\overline{j}q}}
% \newcommand{\tojk}{t_{\overline{j}k}}
% \newcommand{\tojkq}{t_{\overline{jk}q}}
% \newcommand{\tojlq}{t_{\overline{jl}q}}
% \newcommand{\toqc}{t_{\overline{q}c}}
% \newcommand{\tjkq}{t_{j\overline{k}q}}
% \newcommand{\tkjq}{t_{k\overline{j}q}}
% \newcommand{\CNq}{C_{\scriptscriptstyle Nq}}
% \newcommand{\CNf}{C_{\scriptscriptstyle Nf}}
% \newcommand{\CNk}{C_{\scriptscriptstyle Nk}}
% \newcommand{\Ckq}{C_{kq}}
% \newcommand{\Ckc}{C_{kc}}
% \newcommand{\Cqc}{C_{qc}}
% \newcommand{\COc}{C_{\scriptscriptstyle \mathcal{O}c}}
% \newcommand{\Iq}{\mathcal{I}_{q}}
% \newcommand{\Ik}{\mathcal{I}_{k}}
% \newcommand{\IkM}{\mathcal{I}_{0k}}
% \newcommand{\Ikk}{\mathcal{I}_{\overline{k}k}}
% \newcommand{\Ekk}{\mathcal{E}_{\overline{k}k}}
% \newcommand{\Elk}{\mathcal{E}_{\overline{l}k}}
% \newcommand{\Ekq}{\mathcal{E}_{\overline{k}q}}
% \newcommand{\Ikq}{\mathcal{I}_{kq}}
% \newcommand{\Ijk}{\mathcal{I}_{jk}}
% \newcommand{\notIkM}{\overline{\mathcal{I}_{0k}}}
% \newcommand{\notIkk}{\overline{\mathcal{I}_{\overline{k}k}}}
% \newcommand{\notEkk}{\overline{\mathcal{E}_{\overline{k}k}}}
% \newcommand{\notIq}{\overline{\mathcal{I}_{q}}}
% \newcommand{\notIk}{\overline{\mathcal{I}_{k}}}
% \newcommand{\Unq}{U_{nq}}
% %\newcommand{\mcG}{\mathcal{G}}
% \newcommand{\mcGjq}{\mathcal{G}_1, t_{jq}}
% \newcommand{\mcGkq}{\mathcal{G}_1, t_{kq}}
% \newcommand{\mcGjk}{\mathcal{G}_1, t_{jk}}
% \newcommand{\Ok}{\mathcal{O}_k}
% \newcommand{\OkM}{\mathcal{O}_{0k}}
% \newcommand{\Ozeta}{\mathcal{O}_{\zeta}}
% \newcommand{\Oq}{\mathcal{O}_q}
% \newcommand{\notOq}{\overline{\mathcal{O}_q}}
% \newcommand{\notOk}{\overline{\mathcal{O}_k}}
% %\newcommand{\TO}{T_{\scriptscriptstyle \mathcal{O}}}
% %\newcommand{\NO}{N_{\scriptscriptstyle \mathcal{O}}}
% %\newcommand{\PNf}{P_{\scriptscriptstyle Nf}}
% % \newcommand{\OmFSR}{\Omega_{\text{\tiny{FSR}}}}
% \newcommand{\Delpsi}{\Delta\psi}
% \newcommand{\Lpsi}{L_{\psi}}
% \newcommand{\tauPsi}{\tau_{\psi}}
% \newcommand{\Lcoup}{L_{\text{coup}}}
% %\newcommand{\gamL}{\gamma_{\scriptscriptstyle L}}
% %\newcommand{\Pc}{P_{th}}
% \newcommand{\mcX}{\mathcal{X}}
% \newcommand{\mcL}{\mathcal{L}}
% \newcommand{\mcM}{\mathcal{M}}
% %\newcommand{\Ne}{N_{e}}
% \newcommand{\mcOi}{\mathcal{O}_{i}}
% %\newcommand{\ket}[1]{|{#1}\rangle}
% %\newcommand{\bra}[1]{\langle {#1}|}
% \newcommand{\expect}[1]{\big \langle {#1} \big \rangle}
% \newcommand{\GM}{G_{\scriptscriptstyle M}}
% \newcommand{\GMj}{G_{\scriptscriptstyle M}^{\scriptscriptstyle (j)}}
% \newcommand{\GLj}{G_{\scriptscriptstyle \mathcal{L}}^{\scriptscriptstyle (j)}}
% \newcommand{\RM}{R_{\scriptscriptstyle M\minus 1}}
% %\newcommand{\RMk}{R_{\scriptscriptstyle M\minus 1}^{\scriptscriptstyle (k)}}
% \newcommand{\DMk}{D_{\scriptscriptstyle M\minus 1}^{\scriptscriptstyle (k)}}
% \newcommand{\DMkM}{D_{\scriptscriptstyle M}^{\scriptscriptstyle (k)}}
% \newcommand{\RMl}{R_{\scriptscriptstyle M\minus 1}^{\scriptscriptstyle (l)}}
% \newcommand{\RMm}{R_{\scriptscriptstyle \mathcal{M}}^{\scriptscriptstyle (m)}}
% \newcommand{\DGo}{D_{\scriptscriptstyle D}^{\scriptscriptstyle (o)}}
% \newcommand{\Dll}{D^{\scriptscriptstyle (l)}}
% \newcommand{\nc}[1]{n^{\scriptscriptstyle (c)}_{\scriptscriptstyle #1}}
% \newcommand{\nm}[1]{n^{\scriptscriptstyle (m)}_{\scriptscriptstyle #1}}
% \newcommand{\nj}[1]{n^{\scriptscriptstyle (j)}_{\scriptscriptstyle #1}}
% \newcommand{\nI}[1]{n^{\scriptscriptstyle (i)}_{\scriptscriptstyle #1}}
% %\newcommand{\niL}{n^{\scriptscriptstyle (i)}_{\scriptscriptstyle L\text{th}}}
% \newcommand{\nlN}{n^{\scriptscriptstyle (l)}_{\scriptscriptstyle N\text{th}}}
% \newcommand{\nnO}{n^{\scriptscriptstyle (n)}_{\scriptscriptstyle O}}
% \newcommand{\nk}[1]{n^{\scriptscriptstyle (k)}_{\scriptscriptstyle #1}}
% \newcommand{\nl}[1]{n^{\scriptscriptstyle (l)}_{\scriptscriptstyle #1}}
% \newcommand{\ii}[1]{i^{\scriptscriptstyle (i)}_{\scriptscriptstyle #1}}
% \newcommand{\Sl}[1]{s^{\scriptscriptstyle (l)}_{\scriptscriptstyle #1}}


% \newcommand{\Nmk}{\mathcal{N}_{\scriptscriptstyle m}^{\scriptscriptstyle (k)}}
% \newcommand{\NMk}{\mathcal{N}_{\scriptscriptstyle M\minus 1}^{\scriptscriptstyle (k)}}
% \newcommand{\Nmnk}{\mathcal{N}_{\scriptscriptstyle MN}^{\scriptscriptstyle (k)}}
% \newcommand{\MMk}{\mathcal{M}_{\scriptscriptstyle M\minus 1}^{\scriptscriptstyle (k)}}
% \newcommand{\MMkM}{\mathcal{M}_{\scriptscriptstyle M}^{\scriptscriptstyle (k)}}
% \newcommand{\Nak}{\mathcal{N}_{a}^{\scriptscriptstyle (k)}}
% \newcommand{\Nbk}{\mathcal{N}_{b}^{\scriptscriptstyle (k)}}
% \newcommand{\Nck}{\mathcal{N}_{c}^{\scriptscriptstyle (k)}}
% \newcommand{\Nxk}{\mathcal{N}_{x}^{\scriptscriptstyle (k)}}
% \newcommand{\Nk}[1]{\mathcal{N}^{\scriptscriptstyle (k)}_{#1}}
% \newcommand{\nD}{n_{\scriptscriptstyle D}}
% \newcommand{\nC}{n_{\scriptscriptstyle C}}
% \newcommand{\nL}{n_{\scriptscriptstyle L}}
% %\newcommand{\niW}{n_{i\scriptscriptstyle W}}
% \newcommand{\pD}{p_{\scriptscriptstyle D}}
% \newcommand{\pC}{p_{\scriptscriptstyle C}}
% \newcommand{\pL}{p_{\scriptscriptstyle L}}
% \newcommand{\PD}{P_{\scriptscriptstyle D}}
% \newcommand{\PDC}{P_{\scriptscriptstyle DC}}
% \newcommand{\PC}{P_{\scriptscriptstyle C}}
% %\newcommand{\pWn}{p_{\scriptscriptstyle W_n}}
% \newcommand{\pCn}{p_{\scriptscriptstyle C_n}}
% \newcommand{\pLn}{p_{\scriptscriptstyle L_n}}
% \newcommand{\kapwW}{\kappa_{w\scriptscriptstyle W}}
% \newcommand{\kapwD}{\kappa_{w\scriptscriptstyle D}}
% %\newcommand{\kapW}{\kappa_{\scriptscriptstyle W}}
% \newcommand{\kapL}{\kappa_{\scriptscriptstyle L}}
% %\newcommand{\kapI}{\kappa_{\scriptscriptstyle I}}
% %\newcommand{\rhoD}{\rho_{\scriptscriptstyle D}}
% %\newcommand{\rhoIS}{\rho_{\scriptscriptstyle IS}}
% %\newcommand{\tci}{t_{ci}}
% %\newcommand{\tli}{t_{li}}
% %\newcommand{\tlk}{t_{lk}}
% %\newcommand{\tji}{t_{ji}}

% \newcommand{\nSAa}{n_{\scriptscriptstyle SA}^{\scriptscriptstyle (a)}}
% \newcommand{\nAa}{n_{\scriptscriptstyle A}^{\scriptscriptstyle (a)}}
% %\newcommand{\nJn}{n_{\scriptscriptstyle J}^{\scriptscriptstyle (n)}}
% \newcommand{\nJ}[1]{n_{\scriptscriptstyle J}^{\scriptscriptstyle (#1)}}



% \newcommand{\nsJ}[1]{n_{s\scriptscriptstyle J}^{\scriptscriptstyle (#1)}}
% \newcommand{\iK}[1]{i_{\scriptscriptstyle K}^{\scriptscriptstyle (#1)}}
% %\newcommand{\nsJnone}{n_{s\scriptscriptstyle J}}
% %\newcommand{\vnJn}{\boldsymbol{n}_{\scriptscriptstyle J}^{\scriptscriptstyle (\boldsymbol{n})}}
% %\newcommand{\vnJ}{\boldsymbol{n}_{\scriptscriptstyle J}}
% %\newcommand{\vJ}{\boldsymbol{J}}
% %\newcommand{\nJm}{n_{\scriptscriptstyle J}^{\scriptscriptstyle (m)}}
% %\newcommand{\nJsup}[1]{n_{\scriptscriptstyle J}^{\scriptscriptstyle (m_{#1})}}
% %\newcommand{\nJsupP}[1]{n_{\scriptscriptstyle J'}^{\scriptscriptstyle (m_{#1})}}
% %\newcommand{\nJsupL}[1]{n_{\scriptscriptstyle J_{#1 L}}^{\scriptscriptstyle (m_{#1})}}
% \newcommand{\nCc}{n_{\scriptscriptstyle C}^{\scriptscriptstyle (c)}}
% \newcommand{\nCcL}{n_{\scriptscriptstyle C_L}^{\scriptscriptstyle (c)}}
% \newcommand{\nEe}{n_{\scriptscriptstyle E}^{\scriptscriptstyle (e)}}
% \newcommand{\Dp}{D_{\scriptscriptstyle P}^{\scriptscriptstyle (\boldsymbol{p})}}
% \newcommand{\Dg}{D_{\scriptscriptstyle G}^{\scriptscriptstyle (\boldsymbol{g})}}
% %\newcommand{\DGn}{D_{\scriptscriptstyle G}^{\scriptscriptstyle (\boldsymbol{n})}}
% \newcommand{\RNn}{R_{\scriptscriptstyle N}^{\scriptscriptstyle (\boldsymbol{n})}}
% \newcommand{\vRNn}{\boldsymbol{R}_{\scriptscriptstyle N}^{\scriptscriptstyle (\boldsymbol{n})}}
% \newcommand{\notRNn}{\overline{R}_{\scriptscriptstyle N}^{\scriptscriptstyle (\boldsymbol{n})}}
% %\newcommand{\notDGn}{\overline{D}_{\scriptscriptstyle G}^{\scriptscriptstyle (\boldsymbol{n})}}
% %\newcommand{\Ds}{D_{\scriptscriptstyle PG}^{\scriptscriptstyle (\mathbf{bd})}}
% \newcommand{\Ds}{\boldsymbol{D}}
% \newcommand{\iKk}{i_{\scriptscriptstyle K}^{\scriptscriptstyle (k)}}
% \newcommand{\viKk}{\boldsymbol{i}_{\scriptscriptstyle K}^{\scriptscriptstyle (\boldsymbol{k})}}
% \newcommand{\ILl}{\mathcal{I}_{\scriptscriptstyle L}^{\scriptscriptstyle (l)}}

% \newcommand{\sM}[1]{s_{\scriptscriptstyle M}^{\scriptscriptstyle (t_{\scriptscriptstyle #1})}}
% %\newcommand{\Sm}[1]{\mathcal{S}_{\scriptscriptstyle #1}^{\scriptscriptstyle (m)}}
% %\newcommand{\Il}[1]{\mathcal{I}_{\scriptscriptstyle #1}^{\scriptscriptstyle (t_{\scriptscriptstyle #1})}}


% \newcommand{\Hsys}{H_{\text{sys}}}
% \newcommand{\Il}[1]{\mathcal{I}_{\scriptscriptstyle #1}}
% \newcommand{\vmcS}[1]{\boldsymbol{\mathcal{S}}_{\scriptscriptstyle \! #1}}
% %\newcommand{\Ssub}[1]{S_{\scriptscriptstyle  #1}}
% \newcommand{\mcSsub}[1]{\mathcal{S}_{\scriptscriptstyle \! #1}}
% \newcommand{\vmcI}[1]{\boldsymbol{\mathcal{I}}_{\scriptscriptstyle \! #1}}
% \newcommand{\Isub}[1]{I_{\scriptscriptstyle \! #1}}
% \newcommand{\mcIsub}[1]{\mathcal{I}_{\scriptscriptstyle \! #1}}
% \newcommand{\mcIsubsup}[2]{\mathcal{I}_{\scriptscriptstyle \! #1}^{\scriptscriptstyle \! #2}}
% \newcommand{\vILl}{\boldsymbol{\mathcal{I}}_{\scriptscriptstyle L}}
% \newcommand{\kapsD}{\kappa_{s\scriptscriptstyle D}}
% \newcommand{\kapnD}{\kappa_{n\scriptscriptstyle D}}
% \newcommand{\kapsS}{\kappa_{s\scriptscriptstyle S}}
% \newcommand{\kapiD}{\kappa_{i\scriptscriptstyle D}}
% \newcommand{\kappP}{\kappa_{p\scriptscriptstyle P}}
% \newcommand{\kapiL}{\kappa_{i\scriptscriptstyle L}}



% \newcommand{\vg}{\boldsymbol{g}}
% \newcommand{\vtg}{\boldsymbol{t_g}}
% \newcommand{\vp}{\boldsymbol{p}}
% \newcommand{\vtp}{\boldsymbol{t_p}}
% \newcommand{\vn}{\boldsymbol{n}}
% \newcommand{\vnsub}[1]{\boldsymbol{n}_{\scriptscriptstyle #1}}
% \newcommand{\vtn}{\boldsymbol{t_n}}
% \newcommand{\vm}{\boldsymbol{m}}
% \newcommand{\vtm}{\boldsymbol{t_m}}
% \newcommand{\vk}{\boldsymbol{k}}
% \newcommand{\vtk}{\boldsymbol{t_k}}
% \newcommand{\vl}{\boldsymbol{l}}
% \newcommand{\vL}{\boldsymbol{L}}
% \newcommand{\vN}{\boldsymbol{N}}
% \newcommand{\vtl}{\boldsymbol{t_l}}
% \newcommand{\vtsub}[1]{\boldsymbol{t}_{\scriptscriptstyle #1}}
% \newcommand{\tlL}{t_{l_{\scriptscriptstyle L}}}
% \newcommand{\mcI}{\mathcal{I}}
% %\newcommand{\mcS}{\mathcal{S}}
% \newcommand{\vtau}{\boldsymbol{\tau}}
% \newcommand{\Pone}{P_{\text{one}}}
% \newcommand{\trace}[1]{\text{Tr}\Big( #1 \Big)}
% \newcommand{\traceS}[1]{\text{Tr}_{\scriptscriptstyle S} \Big( #1 \Big)}
% \newcommand{\rhoIhat}{\hat{\rho}_{\scriptscriptstyle I}}
% \newcommand{\rhoIShat}{\hat{\rho}_{\scriptscriptstyle IS}}
% \newcommand{\rhoShat}{\hat{\rho}_{\scriptscriptstyle S}}
% \newcommand{\QpW}{Q_{p\scriptscriptstyle W}}
% \newcommand{\QiD}{Q_{i\scriptscriptstyle D}}
% \newcommand{\nte}[1]{n^{\scriptscriptstyle (e)}_{\scriptscriptstyle #1}}
% %\newcommand{\Sn}[1]{S^{\scriptscriptstyle (n)}_{\scriptscriptstyle #1}}
% \newcommand{\PR}{P_{\scriptscriptstyle R}}
% \newcommand{\PG}{P_{\scriptscriptstyle G}}
% \newcommand{\tD}{\tau_{\scriptscriptstyle D}}
% \newcommand{\PWL}{P_{\scriptscriptstyle WL}}
% \newcommand{\PWC}{P_{\scriptscriptstyle WC}}
% \newcommand{\PCC}{P_{\scriptscriptstyle CC}}
% \newcommand{\PCCiD}{P_{\scriptscriptstyle CCiD}}
% \newcommand{\PsCiD}{P_{\scriptscriptstyle sCiD}}
% \newcommand{\rhoR}{\rho_{\scriptscriptstyle R}}
% \newcommand{\rhoI}{\rho_{\scriptscriptstyle I}}
% \newcommand{\rhoIC}{\rho_{\scriptscriptstyle IC}}
% \newcommand{\rhoCC}{\rho_{\scriptscriptstyle CC}}
% \newcommand{\rhoDC}{\rho_{\scriptscriptstyle DC}}
% %\newcommand{\rhoD}{\rho_{\scriptscriptstyle D}}
% \newcommand{\mcN}{\mathcal{N}}
% \newcommand{\mcP}{\mathcal{P}}
% \newcommand{\IntK}{I_{\scriptscriptstyle K}}
% \newcommand{\tN}{t_{\scriptscriptstyle N}}
% \newcommand{\mcE}[2]{\mathcal{E}^{\scriptscriptstyle (#2)}_{\scriptscriptstyle #1}}
% \newcommand{\vmcE}[1]{\boldsymbol{\mathcal{E}}_{\scriptscriptstyle \!#1}}
% \newcommand{\nsCc}{n_{s\scriptscriptstyle C}^{\scriptscriptstyle (c)}}
% \newcommand{\nsEe}{n_{s\scriptscriptstyle E}^{\scriptscriptstyle (e)}}
% \newcommand{\nsJp}[1]{n^{\scriptscriptstyle (t_{#1})}_{s\scriptscriptstyle J'}}
% \newcommand{\niJ}[1]{n^{\scriptscriptstyle (t_{#1})}_{i\scriptscriptstyle J}}
% \newcommand{\NsJp}{n_{s\scriptscriptstyle J'}}
% \newcommand{\NiJ}{n_{i\scriptscriptstyle J}}
% \newcommand{\IJJp}{I_{\scriptscriptstyle \!JJ'}}
% \newcommand{\piC}{p_{i\scriptscriptstyle C}}
% \newcommand{\piL}{p_{i\scriptscriptstyle L}}
% \newcommand{\piD}{p_{i\scriptscriptstyle D}}
% \newcommand{\psC}{p_{s\scriptscriptstyle C}}
% \newcommand{\psL}{p_{s\scriptscriptstyle L}}
% \newcommand{\psD}{p_{s\scriptscriptstyle D}}

% \newcommand{\niD}{n_{i\scriptscriptstyle D}}
% \newcommand{\niC}{n_{i\scriptscriptstyle C}}
% \newcommand{\niL}{n_{i\scriptscriptstyle L}}
% \newcommand{\nsD}{n_{s\scriptscriptstyle D}}
% \newcommand{\nsC}{n_{s\scriptscriptstyle C}}
% \newcommand{\nsL}{n_{s\scriptscriptstyle L}}

% \newcommand{\niDhat}{\hat{n}_{i\scriptscriptstyle D}}
% \newcommand{\niChat}{\hat{n}_{i\scriptscriptstyle C}}
% \newcommand{\niLhat}{\hat{n}_{i\scriptscriptstyle L}}
% \newcommand{\nsDhat}{\hat{n}_{s\scriptscriptstyle D}}
% \newcommand{\nsChat}{\hat{n}_{s\scriptscriptstyle C}}
% \newcommand{\nsLhat}{\hat{n}_{s\scriptscriptstyle L}}
% \newcommand{\nDhat}{\hat{n}_{\scriptscriptstyle D}}
% \newcommand{\nChat}{\hat{n}_{\scriptscriptstyle C}}
% \newcommand{\nLhat}{\hat{n}_{\scriptscriptstyle L}}
% \newcommand{\niCt}[1]{n_{i\scriptscriptstyle C}^{\scriptscriptstyle (t_{#1})}}
% \newcommand{\nsCt}[1]{n_{s\scriptscriptstyle C}^{\scriptscriptstyle (t_{#1})}}

% \newcommand{\niCsubp}[2]{{#1}_{i\scriptscriptstyle C}^{\scriptscriptstyle (#2)}}
% \newcommand{\nsCsubp}[2]{{#1}_{s\scriptscriptstyle C}^{\scriptscriptstyle (#2)}}
% \newcommand{\nLsCsubp}[2]{{#1}_{\scriptscriptstyle LsC}^{\scriptscriptstyle (#2)}}
% \newcommand{\nAsCsubp}[2]{{#1}_{\scriptscriptstyle AsC}^{\scriptscriptstyle (#2)}}
% \newcommand{\isubp}[2]{i_{\scriptscriptstyle #1}^{\scriptscriptstyle (#2)}}
% \newcommand{\ssubp}[2]{s_{\scriptscriptstyle #1}^{\scriptscriptstyle (#2)}}
% \newcommand{\Ftot}{F_{\text{tot}}}
% \newcommand{\CnL}{\hat{C}_{n\scriptscriptstyle L}}
% \newcommand{\CnD}{\hat{C}_{n\scriptscriptstyle D}}
% \newcommand{\CsS}{\hat{C}_{s\scriptscriptstyle S}}
% \newcommand{\tL}{t_{\scriptscriptstyle \!L}}
% \newcommand{\DeltR}{\Delta t_{\scriptscriptstyle R}}
% \newcommand{\tauPoff}{\tau_{\scriptscriptstyle \text{off}}}
% \newcommand{\tg}{t_{g}}
% \newcommand{\Thetattg}{\Theta_{\scriptscriptstyle t, \!t_g}}
% \newcommand{\Thetatgt}{\Theta_{\scriptscriptstyle t_g, \!t}}
% \newcommand{\tr}{t_{r}}
% \newcommand{\Thetattr}{\Theta_{\scriptscriptstyle t, \!t_r}}
% \newcommand{\Thetatrt}{\Theta_{\scriptscriptstyle t_r, \!t}}
% \newcommand{\mean}[1]{\langle #1 \rangle}
% \newcommand{\tauF}[2]{\tau_{\scriptscriptstyle #1 #2}}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %% new commands in PhD_project
% %
% \newcommand{\omc}{\omega_{c}}
% \newcommand{\omcc}{\omega_{cc}}

% \newcommand{\omtil}[1]{\tilde{\omega}_{#1}}
% \newcommand{\sP}{s_{p}}
% \newcommand{\sGP}{s_{gp}}
% \newcommand{\DelGP}{\Delta_{gp}}

% \newcommand{\gGI}{g_{gi}}
% \newcommand{\gGS}{g_{gs}}
% \newcommand{\gGP}{g_{gp}}
% \newcommand{\gamGP}{\gamma_{gp}}
% \newcommand{\gamGS}{\gamma_{gs}}
% \newcommand{\gamGI}{\gamma_{gi}}
% \newcommand{\gamI}{\gamma_{i}}
% \newcommand{\gamP}{\gamma_{p}}
% \newcommand{\gamS}{\gamma_{s}}
% \newcommand{\gamL}{\gamma_{L}}
% \newcommand{\gamWS}{\gamma_{\scriptscriptstyle W_{s}}}
% \newcommand{\gamWP}{\gamma_{\scriptscriptstyle W_{p}}}
% \newcommand{\gamWI}{\gamma_{\scriptscriptstyle W_{i}}}

% \newcommand{\delI}{\delta_{i}}
% \newcommand{\delS}{\delta_{s}}
% \newcommand{\delP}{\delta_{p}}
% \newcommand{\delGP}{\delta_{gp}}
% \newcommand{\delGI}{\delta_{gi}}
% \newcommand{\delGS}{\delta_{gs}}
% \newcommand{\aGP}{a_{gp}}
% \newcommand{\aGS}{a_{gs}}
% \newcommand{\aGI}{a_{gi}}
% \newcommand{\aI}{a_{i}}
% \newcommand{\dotaP}{\dot{a}_{p}}
% \newcommand{\dotaI}{\dot{a}_{i}}
% \newcommand{\dotaS}{\dot{a}_{s}}
% \newcommand{\dotaGS}{\dot{a}_{gs}}
% \newcommand{\dotaGI}{\dot{a}_{gi}}
% \newcommand{\dotaGP}{\dot{a}_{gp}}
% \newcommand{\MO}{\mathbf{0}}
% \newcommand{\MVinv}{\mathbf{V^{\text{\tiny{-1}}}}}
% \newcommand{\MV}{\mathbf{V}}
% \newcommand{\vv}{\mathbf{v}}
% \newcommand{\vyout}{\mathbf{y}_{\text{out}}}
% \newcommand{\vyin}{\mathbf{y}_{\text{in}}}
% \newcommand{\MLam}{\mathbf{\Lambda}}
% \newcommand{\MKap}{\mathbf{K}}
% \newcommand{\MD}{\mathbf{D}}
% \newcommand{\MC}{\mathbf{C}}
% \newcommand{\vsout}{\mathbf{s}_{\text{out}}}
% \newcommand{\vsin}{\mathbf{s}_{\text{in}}}
% \newcommand{\MGam}{\mathbf{\Gamma}}
% \newcommand{\MA}{\mathbf{A}}
% \newcommand{\MOmt}{\tilde{\mathbf{\Omega}}}
% \newcommand{\Gamc}{\Gamma_{c}}
% \newcommand{\Gamcc}{\Gamma_{cc}}
% \newcommand{\gamWcc}{\gamma_{\scriptscriptstyle W_{cc}}}

% \newcommand{\phillm}{\phi_{\text{\tiny{2-}}}}
% \newcommand{\phillmdot}{\dot{\phi}_{\text{\tiny{2-}}}}
% \newcommand{\philp}{\phi_{\text{\tiny{1+}}}}
% \newcommand{\philpdot}{\dot{\phi}_{\text{\tiny{1+}}}}
% \newcommand{\phil}{\phi_{\text{\tiny{1}}}}
% \newcommand{\phildot}{\dot{\phi}_{\text{\tiny{1}}}}
% \newcommand{\Ul}{U_{\text{\tiny{1}}}}
% \newcommand{\Uldot}{\dot{U}_{\text{\tiny{1}}}}
% \newcommand{\Pllm}{P_{\text{\tiny{2-}}}}
% \newcommand{\Plp}{P_{\text{\tiny{1+}}}}
% \newcommand{\Ltheta}{L_{\theta}}
% \newcommand{\thetaref}{\theta_{\text{ref}}}
% \newcommand{\kref}{k_{\text{ref}}}
% \newcommand{\oms}{\omega_{\text{s}}}
% \newcommand{\omp}{\omega_{\text{p}}}
% \newcommand{\omi}{\omega_{\text{i}}}
% \newcommand{\Lphi}{L_{\phi}}
% \newcommand{\Lphil}{L_{\phi_1}}
% \newcommand{\Lphill}{L_{\phi_2}}
% \newcommand{\DelSl}{\Delta_{\text{\tiny{S1}}}}
% \newcommand{\Abold}{\mathbf{A}}
% \newcommand{\gamllw}{\gamma_{\text{2w}}}
% \newcommand{\gamlw}{\gamma_{\text{1w}}}
% \newcommand{\phiref}{\phi_{\text{ref}}}
% \newcommand{\phiRT}{\phi_{\text{\tiny{RT}}}}
% \newcommand{\rllc}{r_{\text{\tiny{2}}}^{\text{c}}}
% \newcommand{\rlc}{r_{\text{\tiny{1}}}^{\text{c}}}
% % \newcommand{\omref}{\omega_{\text{ref}}}
% \newcommand{\Pinref}{P_{\text{in}}^{\text{ref}}}
% \newcommand{\Poutref}{P_{\text{out}}^{\text{ref}}}
% \newcommand{\Pfibref}{P_{\text{fib}}^{\text{ref}}}
% \newcommand{\Plasref}{P_{\text{las}}^{\text{ref}}}
% \newcommand{\Pfibin}{P_{\text{fib}}^{\text{in}}}
% \newcommand{\Pfibout}{P_{\text{fib}}^{\text{out}}}
% \newcommand{\Plas}{P_{\text{las}}}
% \newcommand{\gamradsub}{\gamma_{\text{rad}}}
% \newcommand{\Pradsub}{P_{\text{rad}}}
% \newcommand{\Ptot}{P_{\text{tot}}}
% \newcommand{\Pext}{P_{\text{ext}}}
% \newcommand{\Pwg}{P_{\text{wg}}}
% \newcommand{\Qtot}{Q_{\text{tot}}}
% \newcommand{\Qloss}{Q_{\text{loss}}}
% \newcommand{\Tmax}{T_{\text{max}}}
% \newcommand{\Ccon}{C_{\text{con}}}
% %\newcommand{\omc}{\omega_{\text{c}}}
% \newcommand{\lamc}{\lambda_{\text{c}}}
% \newcommand{\gamloss}{\gamma_{\text{\tiny{loss}}}}
% \newcommand{\tM}{t_{\text{\tiny{M}}}}
% \newcommand{\rM}{r_{\text{\tiny{M}}}}
% \newcommand{\gamWc}{\gamma_{\scriptscriptstyle W_{c}}}
% \newcommand{\delc}{\delta_{c}}
% \newcommand{\Ttrans}{\mathbf{T}}
% \newcommand{\Sscat}{\mathbf{S}}
% \newcommand{\dotaCC}{\dot{a}_{cc}}
% \newcommand{\dotaC}{\dot{a}_{c}}
% \newcommand{\aCC}{a_{cc}}
% \newcommand{\aC}{a_{c}}
% \newcommand{\gamllext}{\gamma_{\text{2ext}}}
% \newcommand{\gamcl}{\gamma_{\text{c}_1}}
% \newcommand{\gamlext}{\gamma_{\text{1ext}}}
% \newcommand{\alin}{a_{\text{\tiny{1in}}}}
% \newcommand{\alout}{a_{\text{\tiny{1out}}}}
% \newcommand{\allin}{a_{\text{\tiny{2in}}}}
% \newcommand{\allout}{a_{\text{\tiny{2out}}}}
% \newcommand{\kapl}{\kappa_{1}}
% \newcommand{\clU}{c_{1}^\dag}
% \newcommand{\clD}{c_{1}}
% \newcommand{\cllU}{c_{2}^\dag}
% \newcommand{\cllD}{c_{2}}
% \newcommand{\allkU}{a_{2k}^\dag}
% \newcommand{\allkD}{a_{2k}}
% \newcommand{\alkU}{a_{1k}^\dag}
% \newcommand{\alkD}{a_{1k}}
% \newcommand{\Hclcll}{H_{\text{c}_1-\text{c}_2}}
% \newcommand{\Hwgllcl}{H_{\text{wg2-c}_1}}
% \newcommand{\Hwglcl}{H_{\text{wg1-c}_1}}
% \newcommand{\Hcl}{H_{\text{c}_1}}
% \newcommand{\Hcll}{H_{\text{c}_2}}
% \newcommand{\Hwgl}{H_{\text{wg1}}}
% \newcommand{\Hwgll}{H_{\text{wg2}}}
% \newcommand{\tcav}{t_{\text{cav}}}
% \newcommand{\rcav}{r_{\text{cav}}}
% %\newcommand{\ic}{\text{i}}
% \newcommand{\DelOB}{\Omega_{\text{\tiny{ob}}}}
% \newcommand{\Toff}{T_{\text{off}}}
% \newcommand{\Ton}{T_{\text{on}}}
% %\newcommand{\phieff}{\phi_{\text{eff}}}
% \newcommand{\e}{\text{e}}
% \newcommand{\tCW}{t_{\text{\tiny{CW}}}}
% \newcommand{\rCW}{r_{\text{\tiny{CW}}}}
% \newcommand{\Leff}{L_{\text{eff}}}
% \newcommand{\thetaAAA}{\theta_{111}}
% \newcommand{\thetaAAB}{\theta_{112}}
% \newcommand{\thetaABB}{\theta_{122}}
% \newcommand{\thetaBBB}{\theta_{222}}
% \newcommand{\thetaABA}{\theta_{121}}
% \newcommand{\thetaBAA}{\theta_{211}}
% \newcommand{\thetaBAB}{\theta_{212}}
% \newcommand{\thetaBBA}{\theta_{221}}
% \newcommand{\gambll}{\gamma_{22}}
% \newcommand{\gambl}{\gamma_{21}}
% \newcommand{\gambllC}{\gamma_{22C}}
% \newcommand{\gamblC}{\gamma_{21C}}
% \newcommand{\thetabl}{\theta_{21}}
% \newcommand{\thetabll}{\theta_{22}}
% \newcommand{\thetablll}{\theta_{23}}
% \newcommand{\thetablv}{\theta_{24}}
% \newcommand{\delbll}{\delta_{22}}
% \newcommand{\delbl}{\delta_{21}}
% \newcommand{\abld}{\dot{a}_{21}}
% \newcommand{\ablld}{\dot{a}_{22}}
% \newcommand{\abl}{a_{21}}
% \newcommand{\abll}{a_{22}}
% \newcommand{\sblp}{s_{21+}}
% \newcommand{\sblm}{s_{21-}}
% \newcommand{\sbllp}{s_{22+}}
% \newcommand{\sbllm}{s_{22-}}
% \newcommand{\sblllp}{s_{23+}}
% \newcommand{\sblllm}{s_{23-}}
% \newcommand{\sblvp}{s_{24+}}
% \newcommand{\sblvm}{s_{24-}}
% \newcommand{\sclp}{s_{31+}}
% \newcommand{\gamll}{\gamma_{2}}
% \newcommand{\gaml}{\gamma_{1}}
% \newcommand{\gamllC}{\gamma_{2C}}
% \newcommand{\gamlC}{\gamma_{1C}}
% \newcommand{\delll}{\delta_{2}}
% \newcommand{\dell}{\delta_{1}}
% \newcommand{\thetal}{\theta_{1}}
% \newcommand{\thetall}{\theta_{2}}
% \newcommand{\thetalll}{\theta_{3}}
% \newcommand{\thetalv}{\theta_{4}}
% \newcommand{\tll}{t_{2}}
% \newcommand{\rll}{r_{2}}
% \newcommand{\tl}{t_{1}}
% \newcommand{\rl}{r_{1}}
% \newcommand{\taCW}{t_{1\text{\tiny{CW}}}}
% \newcommand{\TaCW}{T_{1\text{\tiny{CW}}}}
% \newcommand{\thetaal}{\theta_{11}}
% \newcommand{\thetaall}{\theta_{12}}
% \newcommand{\thetaalll}{\theta_{13}}
% \newcommand{\thetaalv}{\theta_{14}}
% \newcommand{\neff}{n_{\text{eff}}}
% %\newcommand{\tL}{t_{L}}
% \newcommand{\tall}{t_{12}}
% \newcommand{\rall}{r_{12}}
% \newcommand{\tal}{t_{11}}
% \newcommand{\ral}{r_{11}}
% \newcommand{\dal}{d_{111}}
% \newcommand{\dall}{d_{121}}
% \newcommand{\dalll}{d_{131}}
% \newcommand{\dalv}{d_{141}}
% \newcommand{\gamall}{\gamma_{12}}
% \newcommand{\gamal}{\gamma_{11}}
% \newcommand{\gamallC}{\gamma_{12C}}
% \newcommand{\gamalC}{\gamma_{11C}}
% \newcommand{\delall}{\delta_{12}}
% \newcommand{\delal}{\delta_{11}}
% \newcommand{\aald}{\dot{a}_{11}}
% \newcommand{\aalld}{\dot{a}_{12}}
% \newcommand{\aal}{a_{11}}
% \newcommand{\aall}{a_{12}}
% \newcommand{\salp}{s_{11+}}
% \newcommand{\salm}{s_{11-}}
% \newcommand{\sallp}{s_{12+}}
% \newcommand{\sallm}{s_{12-}}
% \newcommand{\salllp}{s_{13+}}
% \newcommand{\salllm}{s_{13-}}
% \newcommand{\salvp}{s_{14+}}
% \newcommand{\salvm}{s_{14-}}
% \newcommand{\Omrep}{\Omega_{\text{rep}}}
% \newcommand{\Ibeat}{I_{\text{beat}}}
% \newcommand{\Is}{I_{\text{s}}}
% \newcommand{\Ic}{I_{\text{c}}}
% \newcommand{\Idc}{I_{\text{dc}}}
% \newcommand{\soN}{s_{n}^{\text{o}}}
% \newcommand{\fOml}{f_{\Omega_1}}
% \newcommand{\fiS}{f_{\text{\tiny{S}}}^{\text{i}}}
% \newcommand{\siN}{s_{n}^{\text{i}}}
% \newcommand{\delSP}{\delta_{\text{\tiny{SP}}}}
% % \newcommand{\si}{s^{\text{i}}}
% \newcommand{\TDel}{T_{\Delta}}
% \newcommand{\LLI}{L_{\text{\tiny{LI}}}}
% \newcommand{\DelOm}{\Delta\Omega}
% \newcommand{\Trep}{T_{\text{rep}}}
% \newcommand{\fout}{f_{\text{out}}}
% \newcommand{\Ucav}{U_{\text{cav}}}
% \newcommand{\DelP}{\Delta_{\text{\tiny{P}}}}
% \newcommand{\sigmaFCA}{\sigma_{\text{\tiny{FCA}}}}
% \newcommand{\betaTPA}{\beta_{\text{\tiny{TPA}}}}
% \newcommand{\epsFCD}{\epsilon_{\text{\tiny{FCD}}}}
% \newcommand{\epsFCA}{\epsilon_{\text{\tiny{FCA}}}}
% \newcommand{\UPf}{U_{\text{\tiny{P\emph{f}}}}}
% \newcommand{\UPi}{U_{\text{\tiny{P\emph{i}}}}}
% \newcommand{\SPD}{S_{\text{\tiny{PD}}}}
% \newcommand{\IPD}{I_{\text{\tiny{PD}}}}
% \newcommand{\InPD}{I_{n}^{\text{\tiny{PD}}}}
% \newcommand{\SL}{S_{\text{\tiny{L}}}}
% \newcommand{\OmMod}{\Omega_{\text{mod}}}
% \newcommand{\Gamrep}{\Gamma_{\text{rep}}}
% \newcommand{\TUmax}{T_{\text{\tiny{U}}}^{\text{max}}}
% \newcommand{\TUmin}{T_{\text{\tiny{U}}}^{\text{min}}}
% \newcommand{\TUon}{T_{\text{\tiny{U}}}^{\text{on}}}
% \newcommand{\TUoff}{T_{\text{\tiny{U}}}^{\text{off}}}
% \newcommand{\OmSP}{\Omega_{\text{\tiny{S/P}}}}
% \newcommand{\delNLal}{\delta_{\text{\tiny{NL}}}^{11}}
% \newcommand{\delNLbl}{\delta_{\text{\tiny{NL}}}^{21}}
% \newcommand{\delNLall}{\delta_{\text{\tiny{NL}}}^{12}}
% \newcommand{\delNLbll}{\delta_{\text{\tiny{NL}}}^{22}}
% \newcommand{\delNLmin}{\delta_{\text{\tiny{NL}}}^{\text{min}}}
% \newcommand{\delSmin}{\delta_{\text{\tiny{S}}}^{\text{min}}}
% \newcommand{\delNL}{\delta_{\text{\tiny{NL}}}}
% \newcommand{\gamNL}{\gamma_{\text{\tiny{NL}}}}
% \newcommand{\gamNLal}{\gamma_{\text{\tiny{NL}}}^{11}}
% \newcommand{\gamNLbl}{\gamma_{\text{\tiny{NL}}}^{21}}
% \newcommand{\gamNLall}{\gamma_{\text{\tiny{NL}}}^{12}}
% \newcommand{\gamNLbll}{\gamma_{\text{\tiny{NL}}}^{22}}
% \newcommand{\Csw}{C_{\text{switch}}}
% \newcommand{\CswMax}{C_{\text{switch}}^{\text{max}}}
% \newcommand{\UoSoff}{U_{\text{\tiny{So}}}^{\text{off}}}
% \newcommand{\UoSon}{U_{\text{\tiny{So}}}^{\text{on}}}
% \newcommand{\UoSrel}{\partial U_{\text{\tiny{S}}}^{\text{o}}}
% \newcommand{\USl}{U_{\text{\tiny{So}}}^{\text{\tiny{0\{1\}}}}}
% \newcommand{\USo}{U_{\text{\tiny{So}}}^{\text{\tiny{1\{0\}}}}}
% \newcommand{\UiSo}{U_{\text{\tiny{Si}}}^{\text{\tiny{1\{0\}}}}}
% \newcommand{\deltP}{\Delta t_{\text{\tiny{P}}}}
% \newcommand{\deltS}{\Delta t_{\text{\tiny{S}}}}
% \newcommand{\deltSP}{\Delta t_{\text{\tiny{S/P}}}}
% \newcommand{\Vjk}{V_{jk}}
% \newcommand{\Plo}{P_{\text{1}}^{\text{o}}}
% \newcommand{\Pllo}{P_{\text{2}}^{\text{o}}}
% %\newcommand{\mytimes}{\!\times\!}
% \newcommand{\rb}{r_{\text{b}}}
% \newcommand{\rC}{r_{\text{\tiny{C}}}}
% \newcommand{\QC}{Q_{\text{\tiny{C}}}}
% \newcommand{\QCl}{Q_{\text{\tiny{C1}}}}
% \newcommand{\QCll}{Q_{\text{\tiny{C2}}}}
% \newcommand{\Qloaded}{Q_{\text{l}}}
% \newcommand{\Qunloaded}{Q_{\text{ul}}}
% \newcommand{\Qbot}{Q_{\bot}}
% \newcommand{\Pin}{P_{\text{in}}}
% \newcommand{\Penv}{P_{\text{env}}}
% \newcommand{\omt}{\tilde{\omega}}
% \newcommand{\NP}{N_{\text{\tiny{P}}}}
% %\newcommand{\vg}{v_\text{g}}
% \newcommand{\ntilde}{\tilde{n}}
% \newcommand{\delL}{\delta_{\text{\tiny{L}}}}
% \newcommand{\delSmax}{\delta_{\text{\tiny{S}}}^{\text{max}}}
% \newcommand{\delPmax}{\delta_{\text{\tiny{P}}}^{\text{max}}}
% \newcommand{\kGamM}{k_{\text{\tiny{$\Gamma$M}}}}
% \newcommand{\tB}{t_{\text{\tiny{B}}}}
% %\newcommand{\equal}{\!=\!}
% \newcommand{\TCW}{T_{\text{\tiny{CW}}}}
% \newcommand{\TU}{T_{\text{\tiny{U}}}}
% \newcommand{\TUF}{T_{\text{\tiny{U}}}^{\text{\tiny{F}}}}
% \newcommand{\TP}{T_{\text{\tiny{P}}}}
% \newcommand{\acos}{\text{acos}}
% \newcommand{\asin}{\text{asin}}
% \newcommand{\myint}[2]{\int_{#1}^{#2} \!\!\!}
% \newcommand{\Tdrop}{T_{\text{drop}}}
% \newcommand{\Tbus}{T_{\text{bus}}}
% \newcommand{\Lamt}{\tilde{\Lambda}}
% \newcommand{\CS}{C_{\text{\tiny{S}}}}
% \newcommand{\Tfil}{T_{\text{fil}}}
% \newcommand{\TF}{T_{\text{\tiny{F}}}}
% \newcommand{\Tcoup}{T_{\text{coup}}}
% \newcommand{\frep}{f_{\text{rep}}}
% \newcommand{\lamC}{\lambda_{\text{\tiny{C}}}}
% \newcommand{\lamS}{\lambda_{\text{\tiny{S}}}}
% \newcommand{\lamF}{\lambda_{\text{\tiny{F}}}}
% \newcommand{\lamP}{\lambda_{\text{\tiny{P}}}}
% \newcommand{\DellamP}{\Delta\lambda_{\text{\tiny{P}}}}
% \newcommand{\DellamS}{\Delta\lambda_{\text{\tiny{S}}}}
% \newcommand{\DellamF}{\Delta\lambda_{\text{\tiny{F}}}}
% \newcommand{\Ktauwg}{K_{\tau_{\text{wg}}}}
% \newcommand{\KdiffNll}{K_{\text{diffN2}}}
% \newcommand{\gam}{\gamma}
% \newcommand{\gamc}{\gamma_{c}}
% \newcommand{\gamcc}{\gamma_{cc}}
% \newcommand{\gamC}{\gamma_{\text{\tiny{C}}}}
% \newcommand{\gamnr}{\gamma_{\text{nr}}}
% \newcommand{\gamLoss}{\gamma_{\text{loss}}}
% \newcommand{\gamdiff}{\gamma_{\text{diff}}}
% \newcommand{\feps}{f_{\epsilon}}
% \newcommand{\qdd}{\ddot{q}}
% \newcommand{\qd}{\dot{q}}
% \newcommand{\ud}{\dot{u}}
% \newcommand{\xcav}{x_{\text{cav}}}
% \newcommand{\ycav}{y_{\text{cav}}}
% \newcommand{\lcav}{l_{\text{cav}}}
% %\newcommand{\TF}{T_{\text{\tiny{F}}}}
% \newcommand{\rUi}{r_{\text{\tiny{U}}}^{\text{i}}}
% \newcommand{\tS}{t_{\text{\tiny{S}}}}
% \newcommand{\tP}{t_{\text{\tiny{P}}}}
% \newcommand{\Kwg}{K_{\text{wg}}}
% \newcommand{\UoS}{U_{\text{\tiny{S}}}^{\text{o}}}
% \newcommand{\UoP}{U_{\text{\tiny{P}}}^{\text{o}}}
% \newcommand{\deltaS}{\delta_{\text{\tiny{S}}}}
% \newcommand{\deltaP}{\delta_{\text{\tiny{P}}}}
% \newcommand{\US}{U_{\text{\tiny{S}}}}
% \newcommand{\UP}{U_{\text{\tiny{P}}}}
% \newcommand{\UPdot}{\dot{U}_{\text{\tiny{P}}}}
% \newcommand{\UC}{U_{\text{\tiny{C}}}}
% \newcommand{\Ull}{U_{11}}
% \newcommand{\DUP}{\Delta_{U_{\text{\tiny{P}}}}}
% \newcommand{\USd}{\dot{U}_{\text{\tiny{S}}}}
% \newcommand{\UPd}{\dot{U}_{\text{\tiny{P}}}}
% \newcommand{\phiS}{\phi_{\text{\tiny{S}}}}
% \newcommand{\phiP}{\phi_{\text{\tiny{P}}}}
% \newcommand{\phiPdot}{\dot{\phi}_{\text{\tiny{P}}}}
% \newcommand{\phiSd}{\dot{\phi}_{\text{\tiny{S}}}}
% \newcommand{\phiPd}{\dot{\phi}_{\text{\tiny{P}}}}
% \newcommand{\phiiP}{\phi_{\text{\tiny{P}}}^{\text{i}}}
% \newcommand{\DphiiP}{\Delta\phi_{\text{\tiny{P}}}^{\text{i}}}
% \newcommand{\phiiS}{\phi_{\text{\tiny{S}}}^{\text{i}}}
% \newcommand{\DphiiS}{\Delta\phi_{\text{\tiny{S}}}^{\text{i}}}
% \newcommand{\PiP}{P_{\text{\tiny{P}}}^{\text{i}}}
% \newcommand{\PiPO}{P_{\text{\tiny{P}}}^{\text{0}}}
% \newcommand{\PiSO}{P_{\text{\tiny{S}}}^{\text{0}}}
% %\newcommand{\siP}{s_{\text{\tiny{P}}}^{\text{i}}}
% %\newcommand{\siS}{s_{\text{\tiny{S}}}^{\text{i}}}
% \newcommand{\PiPt}{\tilde{P}_{\text{\tiny{P}}}^{\text{i}}}
% \newcommand{\FiP}{F_{\text{\tiny{P}}}^{\text{i}}}
% \newcommand{\FiPd}{\dot{F}_{\text{\tiny{P}}}^{\text{i}}}
% \newcommand{\PiS}{P_{\text{\tiny{S}}}^{\text{i}}}
% \newcommand{\PiSt}{\tilde{P}_{\text{\tiny{S}}}^{\text{i}}}
% \newcommand{\UiP}{U_{\text{\tiny{P}}}^{\text{i}}}
% \newcommand{\UiPmin}{U_{\text{\tiny{Pi}}}^{\text{min}}}
% \newcommand{\UiS}{U_{\text{\tiny{S}}}^{\text{i}}}
% \newcommand{\PoP}{P_{\text{\tiny{P}}}^{\text{o}}}
% %\newcommand{\PoPO}{P_{\text{\tiny{P}}}^{0}}
% %\newcommand{\PoPO}{P_{\text{\tiny{P}}}^{0}}
% \newcommand{\PoS}{P_{\text{\tiny{S}}}^{\text{o}}}
% \newcommand{\siR}{s_{\text{i}}^{\text{\tiny{R}}}}
% \newcommand{\siI}{s_{\text{i}}^{\text{\tiny{I}}}}
% \newcommand{\siP}{s_{\text{\tiny{P}}}^{\text{i}}}
% \newcommand{\siS}{s_{\text{\tiny{S}}}^{\text{i}}}
% \newcommand{\SiP}{S_{\text{\tiny{P}}}^{\text{i}}}
% \newcommand{\SiS}{S_{\text{\tiny{S}}}^{\text{i}}}
% \newcommand{\soP}{s_{\text{\tiny{P}}}^{\text{o}}}
% \newcommand{\soS}{s_{\text{\tiny{S}}}^{\text{o}}}
% \newcommand{\aS}{a_{\text{\tiny{S}}}}
% \newcommand{\aP}{a_{\text{\tiny{P}}}}
% \newcommand{\aPdot}{\dot{a}_{\text{\tiny{P}}}}
% \newcommand{\aPR}{a_{\text{\tiny{P}}}^{\text{\tiny{R}}}}
% \newcommand{\aPI}{a_{\text{\tiny{P}}}^{\text{\tiny{I}}}}
% \newcommand{\AS}{A_{\text{\tiny{S}}}}
% \newcommand{\AP}{A_{\text{\tiny{P}}}}
% \newcommand{\KLA}{K_{\text{\tiny{LA}}}}
% \newcommand{\KLAepsI}{K_{\text{\tiny{LA}}}^{\epsilon_{\text{\tiny{I}}}}}
% \newcommand{\KLAdelepsI}{K_{\text{\tiny{LA}}}^{\Delta\epsilon_{\text{\tiny{I}}}}}
% \newcommand{\KTPA}{K_{\text{\tiny{TPA}}}}
% \newcommand{\KcarR}{K_{\text{car}}^{\text{\tiny{R}}}}
% \newcommand{\KcarI}{K_{\text{car}}^{\text{\tiny{I}}}}
% \newcommand{\KTPR}{K_{\text{\tiny{TP}}}^{\text{\tiny{R}}}}
% \newcommand{\KTPI}{K_{\text{\tiny{TP}}}^{\text{\tiny{I}}}}
% \newcommand{\PKerr}{P_{\text{\tiny{Kerr}}}}
% \newcommand{\UKerr}{U_{\text{\tiny{Kerr}}}}
% \newcommand{\KKerr}{K_{\text{\tiny{Kerr}}}}
% \newcommand{\KlKl}{K_{\text{\tiny{Kerr}}}^{\text{\tiny{11}}}}
% \newcommand{\KlKll}{K_{\text{\tiny{Kerr}}}^{\text{\tiny{12}}}}
% \newcommand{\KllKl}{K_{\text{\tiny{Kerr}}}^{\text{\tiny{21}}}}
% \newcommand{\KllKll}{K_{\text{\tiny{Kerr}}}^{\text{\tiny{22}}}}
% \newcommand{\KlTPl}{K_{\text{\tiny{TP}}}^{\text{\tiny{11}}}}
% \newcommand{\KlTPll}{K_{\text{\tiny{TP}}}^{\text{\tiny{12}}}}
% \newcommand{\KllTPl}{K_{\text{\tiny{TP}}}^{\text{\tiny{21}}}}
% \newcommand{\KllTPll}{K_{\text{\tiny{TP}}}^{\text{\tiny{22}}}}
% \newcommand{\KlFCDl}{K_{\text{\tiny{FCD}}}^{\text{\tiny{11}}}}
% \newcommand{\KlFCDll}{K_{\text{\tiny{FCD}}}^{\text{\tiny{12}}}}
% \newcommand{\KllFCDl}{K_{\text{\tiny{FCD}}}^{\text{\tiny{21}}}}
% \newcommand{\KllFCDll}{K_{\text{\tiny{FCD}}}^{\text{\tiny{22}}}}
% \newcommand{\KlFCAl}{K_{\text{\tiny{FCA}}}^{\text{\tiny{11}}}}
% \newcommand{\KlFCAll}{K_{\text{\tiny{FCA}}}^{\text{\tiny{12}}}}
% \newcommand{\KllFCAl}{K_{\text{\tiny{FCA}}}^{\text{\tiny{21}}}}
% \newcommand{\KllFCAll}{K_{\text{\tiny{FCA}}}^{\text{\tiny{22}}}}
% \newcommand{\KjKk}{K_{\text{\tiny{Kerr}}}^{jk}}
% \newcommand{\KjKj}{K_{\text{\tiny{Kerr}}}^{jj}}
% \newcommand{\KjTPk}{K_{\text{\tiny{TP}}}^{jk}}
% %\newcommand{\KlKl}{K_{11}}
% %\newcommand{\KlKll}{K_{12}}
% %\newcommand{\KllKll}{K_{22}}
% %\newcommand{\KllKl}{K_{21}}
% \newcommand{\KTP}{K_{\text{\tiny{TP}}}}
% \newcommand{\KFCD}{K_{\text{\tiny{FCD}}}}
% \newcommand{\KFCA}{K_{\text{\tiny{FCA}}}}
% \newcommand{\zetaNl}{\zeta_{\text{\tiny{N}}_{\!1}}}
% \newcommand{\fNll}{f_{N_2}}
% \newcommand{\fNl}{f_{N_1}}
% \newcommand{\Omcar}{\Omega_{\text{car}}}
% \newcommand{\OmcarR}{\Omega_{\text{car}}^{\text{\tiny{R}}}}
% \newcommand{\OmcarI}{\Omega_{\text{car}}^{\text{\tiny{I}}}}
% \newcommand{\OmTPR}{\Omega_{\text{\tiny{TP}}}^{\text{\tiny{R}}}}
% \newcommand{\OmTPI}{\Omega_{\text{\tiny{TP}}}^{\text{\tiny{I}}}}
% \newcommand{\OmTP}{\tilde{\Omega}_{\text{\tiny{TP}}}}
% \newcommand{\OmS}{\Omega_{\text{\tiny{S}}}}
% \newcommand{\OmP}{\Omega_{\text{\tiny{P}}}}
% \newcommand{\Omj}{\Omega_{\text{j}}}
% \newcommand{\lwg}{l_{\text{wg}}}
% \newcommand{\rwg}{r_{\text{wg}}}
% \newcommand{\rwgl}{r_{\text{wg1}}}
% \newcommand{\rwgll}{r_{\text{wg2}}}
% \newcommand{\vnu}{\boldsymbol{\nu}}
% \newcommand{\vlam}{\boldsymbol{\lambda}}
% \newcommand{\vbeta}{\boldsymbol{\beta}}
% \newcommand{\vgam}{\boldsymbol{\gamma}}
% \newcommand{\veta}{\boldsymbol{\eta}}
% \newcommand{\vs}{\mathbf{s}}
% \newcommand{\vq}{\mathbf{q}}
% \newcommand{\vqd}{\dot{\mathbf{q}}}
% \newcommand{\vqdd}{\ddot{\mathbf{q}}}
% \newcommand{\vkl}{\mathbf{k}^{\text{\tiny{(1)}}}}
% \newcommand{\vkO}{\mathbf{k}^{\text{\tiny{(0)}}}}
% \newcommand{\omlepsr}{\omega_{\epsilon_{\text{r}}}^{\text{\tiny{(1)}}}}
% \newcommand{\omlepsI}{\omega_{\epsilon_{\text{\tiny{I}}}}^{\text{\tiny{(1)}}}}
% \newcommand{\omlepsR}{\omega_{\epsilon_{\text{\tiny{R}}}}^{\text{\tiny{(1)}}}}
% \newcommand{\omlTPA}{\omega_{\text{\tiny{TPA}}}^{\text{\tiny{(1)}}}}
% \newcommand{\omlKerr}{\omega_{\text{\tiny{Kerr}}}^{\text{\tiny{(1)}}}}
% \newcommand{\UllKerr}{U_{\text{\tiny{11}}}^{\text{\tiny{Kerr}}}}
% \newcommand{\UllTPA}{U_{\text{\tiny{11}}}^{\text{\tiny{TPA}}}}
% \newcommand{\delomfil}{\Delta\omega_{\text{fil}}}
% \newcommand{\delomC}{\Delta\omega_{\text{\tiny{C}}}}
% \newcommand{\delomS}{\Delta\omega_{\text{\tiny{S}}}}
% \newcommand{\delomP}{\Delta\omega_{\text{\tiny{P}}}}
% \newcommand{\deloml}{\Delta\omega_{1}}
% \newcommand{\delomll}{\Delta\omega_{2}}
% \newcommand{\delomN}{\Delta\omega_n}
% \newcommand{\omfil}{\omega_{\text{fil}}}
% \newcommand{\omO}{\omega^{\text{\tiny{(0)}}}}
% \newcommand{\oml}{\omega^{\text{\tiny{(1)}}}}
% \newcommand{\omtO}{\tilde{\omega}^{\text{\tiny{(0)}}}}
% \newcommand{\omtl}{\tilde{\omega}^{\text{\tiny{(1)}}}}
% \newcommand{\omaO}{\omega_1^{\text{\tiny{(0)}}}}
% \newcommand{\omal}{\omega_1^{\text{\tiny{(1)}}}}
% \newcommand{\ombO}{\omega_2^{\text{\tiny{(0)}}}}
% \newcommand{\ombl}{\omega_2^{\text{\tiny{(1)}}}}
% \newcommand{\omjl}{\omega_j^{\text{\tiny{(1)}}}}
% \newcommand{\omjO}{\omega_j^{\text{\tiny{(0)}}}}
% \newcommand{\omtaO}{\tilde{\omega}_1^{\text{\tiny{(0)}}}}
% \newcommand{\omtal}{\tilde{\omega}_1^{\text{\tiny{(1)}}}}
% \newcommand{\omtbO}{\tilde{\omega}_2^{\text{\tiny{(0)}}}}
% \newcommand{\omtbl}{\tilde{\omega}_2^{\text{\tiny{(1)}}}}
% \newcommand{\omtjl}{\tilde{\omega}_j^{\text{\tiny{(1)}}}}
% \newcommand{\omtjO}{\tilde{\omega}_j^{\text{\tiny{(0)}}}}
% \newcommand{\mN}{\mathcal{N}}
% %\newcommand{\nc}{\tilde{n}^{\text{\tiny{(3)}}}}
% \newcommand{\ncR}{n_{\text{\tiny{R}}}^{\text{\tiny{(3)}}}}
% \newcommand{\ncI}{n_{\text{\tiny{I}}}^{\text{\tiny{(3)}}}}
% \newcommand{\nR}{n_{\text{\tiny{R}}}}
% %\newcommand{\nI}{n_{\text{\tiny{I}}}}
% \newcommand{\delepsr}{\Delta\epsilon_{\text{r}}}
% \newcommand{\delepsR}{\Delta\epsilon_{\text{\tiny{R}}}}
% \newcommand{\delepsI}{\Delta\epsilon_{\text{\tiny{I}}}}
% \newcommand{\epsR}{\epsilon_{\text{\tiny{R}}}}
% \newcommand{\epsI}{\epsilon_{\text{\tiny{I}}}}
% %%%\newcommand{\Umeana}{\langle U_1 \rangle}
% \newcommand{\Umeanb}{\langle U_2 \rangle}
% \newcommand{\vkap}{\varkappa}
% \newcommand{\vkapH}{\varkappa_{\text{\tiny{H}}}}
% \newcommand{\vkapNH}{\varkappa_{\text{\tiny{NH}}}}
% \newcommand{\tauLA}{\tau_{\text{\tiny{LA}}}}
% \newcommand{\tauPH}{\tau_{\text{ph}}}
% \newcommand{\tauRiseP}{\tau_{\text{\tiny{P}}}^{\text{r}}}
% \newcommand{\tauFallP}{\tau_{\text{\tiny{P}}}^{\text{f}}}
% \newcommand{\tauRiseS}{\tau_{\text{\tiny{S}}}^{\text{r}}}
% \newcommand{\tauFallS}{\tau_{\text{\tiny{S}}}^{\text{f}}}
% \newcommand{\tauabs}{\tau_{\text{abs}}}
% \newcommand{\taudiff}{\tau_{\text{diff}}}
% \newcommand{\tautot}{\tau_{\text{tot}}}
% \newcommand{\taudiffinv}{\tau_{\text{diff\_inv}}}
% \newcommand{\taunr}{\tau_{\text{nr}}}
% \newcommand{\gamwg}{\gamma_{\text{wg}}}
% \newcommand{\gamLA}{\gamma_{\text{\tiny{LA}}}}
% \newcommand{\Gamabs}{\Gamma_{\text{abs}}}
% \newcommand{\GamLA}{\Gamma_{\text{\tiny{LA}}}}
% \newcommand{\GamC}{\Gamma_{\text{\tiny{C}}}}
% \newcommand{\GamF}{\Gamma_{\text{\tiny{F}}}}
% \newcommand{\tGamabs}{\tilde{\Gamma}_{\text{abs}}}
% \newcommand{\tGamLA}{\tilde{\Gamma}_{\text{\tiny{LA}}}}
% \newcommand{\alphaLA}{\alpha_{\text{\tiny{LA}}}}
% \newcommand{\alphaTPA}{\alpha_{\text{\tiny{TPA}}}}
% \newcommand{\KaN}{K_a^{\text{\tiny{$N$}}}}
% \newcommand{\KN}{K_{\text{\tiny{$N$}}}}
% \newcommand{\KNC}{K_{\text{\tiny{$N$C}}}}
% \newcommand{\Nss}{N_{\text{ss}}}
% \newcommand{\Ntr}{N_{\text{tr}}}
% \newcommand{\epsr}{\epsilon_{\text{r}}}
% \newcommand{\epsB}{\epsilon_{\text{\tiny{B}}}}
% \newcommand{\epsrmax}{\epsilon_{\text{r}}^{\text{max}}}
% \newcommand{\sigmaFC}{\sigma_{\text{\tiny{FC}}}}
% %\newcommand{\betaTPA}{\beta_{\text{\tiny{TPA}}}}
% \newcommand{\Vcar}{V_{\text{car}}}
% %\newcommand{\Vcarl}{V_{\text{car1}}}
% %\newcommand{\Vcarll}{V_{\text{car2}}}
% \newcommand{\Vcarl}{V_1}
% \newcommand{\Vcarll}{V_2}
% \newcommand{\Vcav}{V_{\text{cav}}}
% \newcommand{\Tcav}{T_{\text{cav}}}
% \newcommand{\IVcar}{I_{V_{\text{car}}}}
% \newcommand{\omL}{\omega_{\text{\tiny{L}}}}
% \newcommand{\omS}{\omega_{\text{\tiny{S}}}}
% \newcommand{\omF}{\omega_{\text{\tiny{F}}}}
% \newcommand{\omP}{\omega_{\text{\tiny{P}}}}
% \newcommand{\omR}{\omega_{\text{\tiny{R}}}}
% \newcommand{\omI}{\omega_{\text{\tiny{I}}}}
% \newcommand{\omReff}{\omega_{\text{eff}}^{{\text{\tiny{R}}}}}
% \newcommand{\omIeff}{\omega_{\text{eff}}^{{\text{\tiny{I}}}}}
% %\newcommand{\QC}{Q_{\text{\tiny{C}}}}
% \newcommand{\QLoss}{Q_{\text{loss}}}
% \newcommand{\Qwg}{Q_{\text{wg}}}
% \newcommand{\Qenv}{Q_{\text{env}}}
% \newcommand{\omC}{\omega_{\text{\tiny{C}}}}
% %\newcommand{\acl}{a_{\text{c}}^1}
% %\newcommand{\apl}{a_{\text{p}}^1}
% \newcommand{\aco}{a_{\text{c}}^0}
% \newcommand{\phico}{\phi_{\text{c}}^0}
% \newcommand{\phipo}{\phi_{\text{p}}^0}
% \newcommand{\phicl}{\phi_{\text{c}}^1}
% \newcommand{\phipl}{\phi_{\text{p}}^1}
% \newcommand{\apo}{a_{\text{p}}^0}
% %\newcommand{\ac}{a_{\text{c}}}
% %\newcommand{\ap}{a_{\text{p}}}
% \newcommand{\fNL}{f_{\text{\tiny{NL}}}}
% \newcommand{\sLA}{s_{\text{\tiny{LA}}}}
% \newcommand{\sabs}{s_{\text{abs}}}
% \newcommand{\swg}{s_{\text{wg}}}
% \newcommand{\senv}{s_{\text{env}}}
% \newcommand{\sIn}{s_{\text{in}}}
% \newcommand{\sOut}{s_{\text{out}}}
% \newcommand{\slp}{s_{\scriptscriptstyle 1+}}
% \newcommand{\slm}{s_{\scriptscriptstyle 1-}}
% \newcommand{\sllp}{s_{\scriptscriptstyle 2+}}
% \newcommand{\sllm}{s_{\scriptscriptstyle 2-}}
% \newcommand{\sinc}{s_{1+}^{\text{c}}}
% \newcommand{\sinp}{s_{1+}^{\text{p}}}
% \newcommand{\tauC}{\tau_{\text{\tiny{C}}}}
% \newcommand{\tauCC}{\tau_{\text{\tiny{CC}}}}
% \newcommand{\tauN}{\tau_{\text{\tiny{$N$}}}}
% \newcommand{\tauCH}{\tau_{\text{\tiny{CH}}}}
% \newcommand{\tauwg}{\tau_{\text{wg}}}
% \newcommand{\tauwgl}{\tau_{\text{1wg}}}
% \newcommand{\tauwgll}{\tau_{\text{2wg}}}
% \newcommand{\tauenv}{\tau_{\text{env}}}
% \newcommand{\Tr}[1]{Tr\left(\underline{\underline{#1}}\right)}
% \newcommand{\Det}[1]{Det\left(\underline{\underline{#1}}\right)}
% \newcommand{\uline}[1]{\underline{#1}}
% \newcommand{\uuline}[1]{\underline{\underline{#1}}}
% \newcommand{\ti}[1]{\tilde{#1}}
% \newcommand{\norm}[1]{\langle\langle{#1}\rangle\rangle}
% \newcommand{\Irat}{I_{1/0}}
% \newcommand{\Umean}{\langle U \rangle}
% \newcommand{\Umeani}{\langle U_i \rangle}
% \newcommand{\Umeanj}{\langle U_j \rangle}
% \newcommand{\tildechic}{\tilde{\chi}^{\text{\tiny{(3)}}}}
% \newcommand{\chic}{\chi^{\text{\tiny{(3)}}}}
% %\newcommand{\Vchic}{V_{\chi^{\text{\tiny{(3)}}}}}
% \newcommand{\Vchic}{V_{\chi}}
% \newcommand{\chil}{\chi^{\text{\tiny{(1)}}}}
% \newcommand{\chicI}{\chi_{\text{\tiny{I}}}^{\text{\tiny{(3)}}}}
% \newcommand{\chicR}{\chi_{\text{\tiny{R}}}^{\text{\tiny{(3)}}}}
% \newcommand{\chicmax}{\chi^{(3)}_{\text{max}}}
% \newcommand{\Pc}{P^{(3)}}
% \newcommand{\vPc}{\mathbf{P}^{(3)}}
% \newcommand{\vPcn}{\mathbf{P}_n^{(3)}}
% \newcommand{\vPcns}{\mathbf{P}_n^{(3)*}}
% \newcommand{\mPc}{\mathcal{P}^{(3)}}
% \newcommand{\vmPc}{\vec{\mathcal{P}}^{(3)}}
% \newcommand{\vPcO}{\mathbf{P}_{\omega_0}^{(3)}(\mathbf{r}) }
% \newcommand{\vPcs}{\mathbf{P}^{(3)*}}
% \newcommand{\vE}{\mathbf{E}}
% \newcommand{\vEwg}{\mathbf{E}_{\text{wg}}}
% \newcommand{\vEa}{\mathbf{E}^{\text{\tiny{(0)}}}}
% \newcommand{\vEl}{\mathbf{E}_1}
% \newcommand{\vEn}{\mathbf{E}_n}
% \newcommand{\vEns}{\mathbf{E}_n^*}
% \newcommand{\vHn}{\mathbf{H}_n}
% \newcommand{\vHns}{\mathbf{H}_n^*}
% \newcommand{\vhn}{\mathbf{h}_n}
% \newcommand{\vEls}{\mathbf{E}_1^*}
% \newcommand{\vEla}{\mathbf{E}_1^{\text{\tiny{(0)}}}}
% \newcommand{\vElsa}{\mathbf{E}_1^{\text{\tiny{(0)*}}}}
% \newcommand{\vEb}{\mathbf{E}^{\text{\tiny{(1)}}}}
% \newcommand{\vEll}{\mathbf{E}_2}
% \newcommand{\vElls}{\mathbf{E}_2^*}
% \newcommand{\vElla}{\mathbf{E}_2^{\text{\tiny{(0)}}}}
% \newcommand{\vEllsa}{\mathbf{E}_2^{\text{\tiny{(0)*}}}}
% \newcommand{\vEsa}{\mathbf{E}^{\text{\tiny{(0)*}}}}
% \newcommand{\vEsb}{\mathbf{E}^{\text{\tiny{(1)*}}}}
% \newcommand{\mE}{\mathcal{E}}
% \newcommand{\vmE}{\vec{\mathcal{E}}}
% \newcommand{\vEs}{\mathbf{E}^*}
% \newcommand{\vEO}{\mathbf{E}_{\omega_0}(\mathbf{r})}
% \newcommand{\vEOs}{\mathbf{E}_{\omega_0}^*(\mathbf{r})}
% \newcommand{\vD}{\mathbf{D}}
% \newcommand{\vmD}{\vec{\mathcal{D}}}
% \newcommand{\vP}{\mathbf{P}}
% \newcommand{\vmP}{\vec{\mathcal{P}}}
% \newcommand{\vF}{\mathbf{F}}
% \newcommand{\vG}{\mathbf{G}}
% \newcommand{\vH}{\mathbf{H}}
% \newcommand{\vHa}{\mathbf{H}^{\text{\tiny{(0)}}}}
% \newcommand{\vHl}{\mathbf{H}_a}
% \newcommand{\vHll}{\mathbf{H}_b}
% \newcommand{\vS}{\boldsymbol{S}}
% \newcommand{\mS}{\mathcal{S}}
% \newcommand{\vmS}{\mathbf{\mathcal{S}}}
% \newcommand{\vx}{\mathbf{x}}
% \newcommand{\vy}{\mathbf{y}}
% \newcommand{\vz}{\mathbf{z}}
% \newcommand{\va}{\mathbf{a}}
% \newcommand{\vA}{\mathbf{A}}
% \newcommand{\vC}{\mathbf{C}}
% \newcommand{\vK}{\mathbf{K}}
% \newcommand{\vOm}{\mathbf{\Omega}}
% \newcommand{\vGam}{\mathbf{\Gamma}}
% \newcommand{\vGamPort}{\mathbf{\Gamma}_{\text{port}}}
% \newcommand{\vGamLoss}{\mathbf{\Gamma}_{\text{loss}}}
% %\newcommand{\vk}{\mathbf{k}}
% \newcommand{\vu}{\mathbf{u}}
% \newcommand{\vh}{\mathbf{h}}
% \newcommand{\vnhat}{\hat{\mathbf{n}}}
% \newcommand{\vrhat}{\hat{\mathbf{r}}}
% \newcommand{\vuko}{\mathbf{u}_{\mathbf{k}^{\text{\tiny{(0)}}}}}
% \newcommand{\vas}{\mathbf{a}^*}
% \newcommand{\eminus}{e^{-i\om t}}
% \newcommand{\eplus}{e^{i\om t}}
% \newcommand{\vb}{\mathbf{b}}
% \newcommand{\vfcav}{\mathbf{\tilde{f}}_{\text{\tiny{C}}}}
% \newcommand{\vfn}{\mathbf{\tilde{f}}_n}
% \newcommand{\vfns}{\mathbf{\tilde{f}}_n^*}
% \newcommand{\vfl}{\mathbf{\tilde{f}}_{\text{1}}}
% \newcommand{\vfls}{\mathbf{\tilde{f}}_{\text{1}}^*}
% \newcommand{\vfll}{\mathbf{\tilde{f}}_{\text{2}}}
% \newcommand{\vflls}{\mathbf{\tilde{f}}_{\text{2}}^*}
% \newcommand{\vfj}{\mathbf{\tilde{f}}_{j}}
% \newcommand{\vfjs}{\mathbf{\tilde{f}}_{j}^*}
% \newcommand{\vfk}{\mathbf{\tilde{f}}_{k}}
% \newcommand{\vfks}{\mathbf{\tilde{f}}_{k}^*}
% \newcommand{\vhcav}{\mathbf{\tilde{h}}_{\text{\tiny{C}}}}
% \newcommand{\vft}{\mathbf{\tilde{f}}}
% \newcommand{\vf}{\mathbf{f}}
% \newcommand{\vehat}{\hat{\mathbf{e}}}
% \newcommand{\ve}{\mathbf{e}}
% \newcommand{\vbs}{\mathbf{b}^*}
% \newcommand{\ays}{a_y^*}
% \newcommand{\axs}{a_x^*}
% \newcommand{\ayss}{a_y^{*2}}
% \newcommand{\axss}{a_x^{*2}}
% \newcommand{\bys}{b_y^*}
% \newcommand{\bxs}{b_x^*}
% \newcommand{\byss}{b_y^{*2}}
% \newcommand{\bxss}{b_x^{*2}}
% \newcommand{\nab}{\nabla}
% \newcommand{\intdr}{\int_V \!d\mathbf{r}}
% \newcommand{\Pout}{P_{\text{out}}}
% \newcommand{\Poutmean}{\langle P_{\text{out}}\rangle}
% \newcommand{\Pouti}{P_{\text{out},i}}
% \newcommand{\PoutX}{P_{\text{out}X}}
% \newcommand{\PoutY}{P_{\text{out}Y}}
% \newcommand{\PinX}{P_{\text{in}X}}
% \newcommand{\PinY}{P_{\text{in}Y}}
% \newcommand{\Souti}{S_{\text{out},i}}
% \newcommand{\SoutX}{S_{\text{out}X}}
% \newcommand{\SoutY}{S_{\text{out}Y}}
% \newcommand{\SinX}{S_{\text{in}X}}
% \newcommand{\SinY}{S_{\text{in}Y}}
% \newcommand{\delSoutX}{\Delta S_{\text{out}X}}
% \newcommand{\delSoutY}{\Delta S_{\text{out}Y}}
% \newcommand{\delSinX}{\Delta S_{\text{in}X}}
% \newcommand{\delSinY}{\Delta S_{\text{in}Y}}
% \newcommand{\delPinX}{\Delta P_{\text{in}X}}
% \newcommand{\delPinY}{\Delta P_{\text{in}Y}}
% \newcommand{\delPoutX}{\Delta P_{\text{out}X}}
% \newcommand{\delPoutY}{\Delta P_{\text{out}Y}}
% \newcommand{\delabsSinX}{\Delta |S_{\text{in}X}|}
% \newcommand{\delabsSinY}{\Delta |S_{\text{in}Y}|}
% \newcommand{\delabsAX}{\Delta |A_X|^2}
% \newcommand{\delabsAY}{\Delta |A_Y|^2}
% \newcommand{\souti}{|s_{i_{2-}}|^2}
% \newcommand{\sini}{|s_{i_{1+}}|^2}
% \newcommand{\soutj}{|s_{j_{2-}}|^2}
% \newcommand{\sinj}{|s_{j_{1+}}|^2}
% \newcommand{\Gam}{\Gamma}
% \newcommand{\AXO}{|A_X^0|^2}
% \newcommand{\AYO}{|A_Y^0|^2}

% % Mikkel's Commands
% %\newcommand{\gamenv}{\gamma_{\text{env}}}
% \newcommand{\gamenv}{\gamma_{\bot}}
% \newcommand{\varep}{\varepsilon}
% \newcommand{\ep}{\epsilon}
% \newcommand{\mc}{\mathcal}
% %\newcommand{\mcE}{\mathcal{E}}
% %\newcommand{\vmcE}{\vec{\mathcal{E}}}
% \newcommand{\vmcB}{\vec{\mathcal{B}}}
% \newcommand{\vmcH}{\vec{\mathcal{H}}}
% \newcommand{\vmcM}{\vec{\mathcal{M}}}
% \newcommand{\vmcP}{\vec{\mathcal{P}}}
% \newcommand{\vmcPl}{\vec{\mathcal{P}}^{\text{\tiny{(1)}}}}
% \newcommand{\vmcPc}{\vec{\mathcal{P}}^{\text{\tiny{(3)}}}}
% \newcommand{\vmcD}{\vec{\mathcal{D}}}
% \newcommand{\vmcJ}{\vec{\mathcal{J}}}
% \newcommand{\pa}{\partial}	
% \newcommand{\mbf}{\mathbf}
% \newcommand{\vmc}[1]{\vec{\mc{#1}}}
% \newcommand{\intinf}{\int_{-\infty}^{+\infty}}
% \newcommand{\gq}{\gamma_q}
% \newcommand{\bigint}[2]{\int_{{}_{#1}}^{{}^{#2}}\!\!\!\!\!}
% \newcommand{\pom}{\omega'}
% \newcommand{\Lble}{L_{\mbox{\tiny{$BLE$}}}}
% \newcommand{\nble}{n_{\mbox{\tiny{$BLE$}}}}
% \newcommand{\ngo}{n_{g}^{0}}
% \newcommand{\vgo}{v_{g}^{0}}
% \newcommand{\ngble}{n_{g}^{\mbox{\tiny{$BLE$}}}}
% \newcommand{\vgble}{v_{g}^{\mbox{\tiny{$BLE$}}}}
% \newcommand{\zetaBLE}{\zeta_{\mbox{\tiny{$BLE$}}}}
% \newcommand{\kom}[1]{k_{\omega_0}^{(#1)}}
% \newcommand{\Do}[1]{D_0^{(#1)}}
% \newcommand{\omom}{(\omega-\omega_0)}
% \newcommand{\gain}{g}
% %\newcommand{\om}{\omega}
% \newcommand{\bmcG}{\bar{\mc{G}}}
% \newcommand{\zble}{z_{\mbox{\tiny{$BLE$}}}}
% \newcommand{\zetable}{\zeta_{\mbox{\tiny{$BLE$}}}}
% \newcommand{\Lpcw}{L_{\mbox{\tiny{$PCW$}}}}
% \newcommand{\zpcw}{z_{\mbox{\tiny{$PCW$}}}}
% \newcommand{\ompcw}{\omega_{\mbox{\tiny{$PCW$}}}}
% \newcommand{\Lpcwti}{\tilde{L}_{\mbox{\tiny{$PCW$}}}}
% \newcommand{\Lpcwbar}{\bar{L}_{\mbox{\tiny{$PCW$}}}}
% \newcommand{\ngpcw}{n_{g}^{\mbox{\tiny{$PCW$}}}}
% \newcommand{\vgpcw}{v_{g}^{\mbox{\tiny{$PCW$}}}}
% \newcommand{\Exp}[1]{\cdot10^{#1}}
% %\newcommand{\bra}[1]{\langle #1 |}
% \newcommand{\mbfD}{\mathbf{D}}
% \newcommand{\mbfT}{\mathbf{T}}
% \newcommand{\trm}[1]{\textrm{#1}}
% \newcommand{\Om}{\Omega}
% \newcommand{\Omti}{\tilde{\Omega}}
% \newcommand{\mcDf}{\mathcal{D}_f}
% \newcommand{\delOm}{\Delta\Omega}
% \newcommand{\delom}{\Delta\omega}
% \newcommand{\delomFWHM}{\Delta\omega_{\text{\tiny{FWHM}}}}
% \newcommand{\delOmti}{\Delta\tilde{\Omega}}
% \newcommand{\delomti}{\Delta\tilde{\omega}}
% \newcommand{\deltau}{\Delta\tau}
% \newcommand{\sigmati}{\tilde{\sigma}}
% \newcommand{\Rbar}{\bar{R}}
% \newcommand{\Gbar}{\bar{G}}
% \newcommand{\Qbar}{\bar{Q}}
% \newcommand{\LN}[1]{\mbox{ln}\!\left(#1\right)}
% \newcommand{\mcTo}{\mathcal{T}_0}
% \newcommand{\mcTP}{\mathcal{T}_P}
% \newcommand{\mcT}{\mathcal{T}}
% \newcommand{\PPmean}{\overline{P}_{\text{\tiny{P}}}^{\text{i}}}
% \newcommand{\PSmean}{\overline{P}_{\text{\tiny{S}}}^{\text{i}}} 
% \newcommand{\Pmean}{\langle P \rangle}
% \newcommand{\Pmeanti}{\langle \tilde{P} \rangle}
% \newcommand{\delt}{\Delta t}
% %\newcommand{\deltP}{\Delta t_P}
% %\newcommand{\delomP}{\Delta \omega_P}
% \newcommand{\deltble}{\Delta t_{\mbox{\tiny{$BLE$}}}}
% \newcommand{\deltauble}{\Delta \tau_{\mbox{\tiny{$BLE$}}}}
% \newcommand{\delOmble}{\Delta \omega_{\mbox{\tiny{$BLE$}}}}
% \newcommand{\delOmtible}{\Delta \tilde{\omega}_{\mbox{\tiny{$BLE$}}}}
% \newcommand{\deltpcw}{\Delta t_{\mbox{\tiny{$PCW$}}}}
% \newcommand{\deltaupcw}{\Delta \tau_{\mbox{\tiny{$PCW$}}}}
% \newcommand{\delOmpcw}{\Delta \omega_{\mbox{\tiny{$PCW$}}}}
% \newcommand{\delOmtipcw}{\Delta \tilde{\omega}_{\mbox{\tiny{$PCW$}}}}
% \newcommand{\Nqtr}{N_q^{tr}}
% \newcommand{\ati}{\tilde{a}}
% \newcommand{\mcO}{\mathcal{O}}
% \newcommand{\IM}[1]{\mbox{Im}\!\left\{#1\right\}}
% \newcommand{\RE}[1]{\mbox{Re}\!\left\{#1\right\}}
% \newcommand{\Atan}[1]{\arctan\!\left[#1\right]}
% \newcommand{\COS}[1]{\cos\!\left[#1\right]}
% \newcommand{\SIN}[1]{\sin\!\left[#1\right]}
% \newcommand{\mcH}[1]{\mathcal{H}\left\{#1\right\}}
% \newcommand{\NWg}{N_W^g}
% \newcommand{\NWq}{N_W^q}
% \newcommand{\NbarWg}{n_W^g}
% \newcommand{\NbarWq}{n_W^q}
% \newcommand{\Neg}{N_e^g}
% \newcommand{\fWg}{f_W^g}
% \newcommand{\fWq}{f_W^q}
% \newcommand{\feg}{f_e^g}
% \newcommand{\feq}{f_e^q}
% \newcommand{\fegmax}{\bar{f}_{e,max}^g}
% \newcommand{\feqmax}{\bar{f}_{e,max}^q}
% \newcommand{\ghatg}{\hat{g}_g}
% \newcommand{\ghatq}{\hat{g}_q}
% \newcommand{\rhoGg}{\rho_G^g}
% \newcommand{\rhoGq}{\rho_G^q}
% \newcommand{\rhoWg}{\rho_W^g}
% \newcommand{\rhoWq}{\rho_W^q}
% \newcommand{\taug}{\tau^g}
% \newcommand{\tauq}{\tau^q}
% \newcommand{\tauWg}{\tau_W^g}
% \newcommand{\tauWq}{\tau_W^q}
% \newcommand{\tauCg}{\tau_C^g}
% \newcommand{\tauCq}{\tau_C^q}
% \newcommand{\tauescg}{\tau_{esc}^g}
% \newcommand{\tauescq}{\tau_{esc}^q}
% %\newcommand{\tg}{t^g}
% \newcommand{\tq}{t^q}
% \newcommand{\tWg}{t_W^g}
% \newcommand{\tWq}{t_W^q}
% \newcommand{\tCg}{t_C^g}
% \newcommand{\tCq}{t_C^q}
% \newcommand{\tescg}{t_{esc}^g}
% \newcommand{\tescq}{t_{esc}^q}
% \newcommand{\epsG}{\varepsilon_G}
% \newcommand{\Iog}{I_0^g}
% \newcommand{\Ioq}{I_0^q}
% \newcommand{\fchi}{f_\chi}
% \newcommand{\fchiG}{f_\chi^G}
% \newcommand{\fchiH}{f_\chi^\mathcal{H}}
% \newcommand{\duty}{R_{\deltP}^T}
% \newcommand{\ghatG}{\hat{g}_g}
% \newcommand{\ghatQ}{\hat{g}_q}
% \newcommand{\mcG}{\mathcal{G}}

% \newcommand{\capwidth}{0.9\textwidth}
% \newcommand{\subfigwidth}{0.44\textwidth}
% \newcommand{\figwidth}{0.9\textwidth}
% \newcommand{\plotwidth}{0.46\textwidth}
% \newcommand{\subplotwidth}{0.35\textwidth}

% \newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}
% \newcommand{\clr}{\clearemptydoublepage}

% % SPACINGS
% \newcommand{\linie}{\underline{\makebox[\textwidth]{}}}
% \newcommand{\spacer}{\rule[-2mm]{0mm}{6mm}}
% \newcommand{\notop}{{{}_{}}}
% \newcommand{\ontop}[1]{{{#1}_{}}}
% %
% % LITERAL ABBREVIATIONS
% \newcommand{\ie}{{i.e.}}
% \newcommand{\eg}{{e.g.}}
% \newcommand{\etal}{\textit{et~al.}}
% %
% % MATH SYMBOLS
% \newcommand{\sgn}{\textrm{sgn}}
% \newcommand{\sm}{\!-\!}
% %\newcommand{\sP}{\!+\!}
% \newcommand{\im}{\mathrm{Im}\:{}}
% \newcommand{\re}{\mathrm{Re}\:{}}
% \newcommand{\krondel}[2]{\delta^\notop_{#1 #2}}
% %\newcommand{\Tr}{\textrm{Tr}}
% \newcommand{\ion}{i\omega^\notop_n}
% \newcommand{\taun}{\tau^\notop}
% \newcommand{\lamn}{\lambda^{{}}}
% \newcommand{\gamn}{\gamma^{{}}}
% \newcommand{\nun}{\nu^\notop}
% %\newcommand{\ve}{\varepsilon}
% \newcommand{\ven}{\ve^\notop}
% \newcommand{\xin}{\xi^\notop}
% \newcommand{\pp}{\partial^{{}}}
% \newcommand{\ppsqr}{\partial^{\,2_{}}}
% \newcommand{\nablabf}{\boldsymbol{\nabla}}
% %
% % MATH STYLE
% \newcommand{\scap}{\!\cdot\!}
% \newcommand{\intd}[1]{{\int\!d#1\: }}
% \newcommand{\inttau}[1]{{\int_0^\beta\!d\tauno_{#1}\: }}
% %\newcommand{\bm}[1]{\makebox{\boldmath $#1$}}
% \newcommand{\dpst}{\displaystyle}
% \newcommand{\scst}{\scriptstyle}
% \newcommand{\scscst}{\scriptscriptstyle}
% \newcommand{\fracsmall}[2]{\makebox{\footnotesize $\dpst\frac{#1}{#2}$}}
% \newcommand{\sqrtsmall}[1]{\makebox{\footnotesize $\dpst\sqrt{#1}$}}
% \newcommand{\half}{\fracsmall{1}{2}}
% \newcommand{\third}{\fracsmall{1}{3}}
% \newcommand{\quarter}{\fracsmall{1}{4}}
% %
% % BOLD SYMBOLS
% \newcommand{\AAA}{\mathbf{A}}
% \newcommand{\AAn}{\mathbf{A}^\notop}
% \newcommand{\aaa}{\mathbf{a}}
% \newcommand{\aan}{\mathbf{a}^\notop}
% \newcommand{\BBB}{\mathbf{B}}
% \newcommand{\BBn}{\mathbf{B}^\notop}
% \newcommand{\bbb}{\mathbf{b}}
% \newcommand{\bbn}{\mathbf{b}^\notop}
% \newcommand{\CCC}{\mathbf{C}}
% \newcommand{\CCn}{\mathbf{C}^\notop}
% \newcommand{\DDD}{\mathbf{D}}
% \newcommand{\DDn}{\mathbf{D^\notop}}
% \newcommand{\ddd}{\mathbf{d}}
% \newcommand{\ddn}{\mathbf{d^\notop}}
% \newcommand{\EEE}{\mathbf{E}}
% \newcommand{\EEn}{\mathbf{E^\notop}}
% \newcommand{\eee}{\mathbf{e}}
% \newcommand{\een}{\mathbf{e}^\notop}
% \newcommand{\FFF}{\mathbf{F}}
% \newcommand{\FFn}{\mathbf{F}^\notop}
% \newcommand{\FFFe}{\mathbf{F}^\notop_\textrm{el}}
% \newcommand{\fff}{\mathbf{f}}
% \newcommand{\ffn}{\mathbf{f}^\notop}
% \newcommand{\fffe}{\mathbf{f}^\notop_\textrm{el}}
% \newcommand{\GGn}{\mathbf{G}}
% \newcommand{\GGG}{\mathbf{G}^\notop}
% \newcommand{\ggn}{\mathbf{g}^\notop}
% \newcommand{\JJJ}{\mathbf{J}}
% \newcommand{\JJn}{\mathbf{J}^\notop}
% \newcommand{\JJJe}{\mathbf{J}^\notop_\textrm{el}}
% \newcommand{\kkk}{\mathbf{k}}
% \newcommand{\kkn}{\mathbf{k}^\notop}
% \newcommand{\KKK}{\mathbf{K}}
% \newcommand{\KKn}{\mathbf{K}^\notop}
% \newcommand{\MMM}{\mathbf{M}}
% \newcommand{\MMn}{\mathbf{M}^\notop}
% \newcommand{\nnn}{\mathbf{n}}
% \newcommand{\PPP}{\mathbf{P}}
% \newcommand{\PPn}{\mathbf{P}^\notop}
% \newcommand{\ppp}{\mathbf{p}}
% \newcommand{\ppn}{\mathbf{p}^\notop}
% \newcommand{\QQQ}{\mathbf{Q}}
% \newcommand{\QQn}{\mathbf{Q}^\notop}
% \newcommand{\qqq}{\mathbf{q}}
% \newcommand{\qqn}{\qqq^\notop}
% \newcommand{\RRR}{\mathbf{R}}
% \newcommand{\RRn}{\RRR^\notop}
% \newcommand{\rrr}{\mathbf{r}}
% \newcommand{\rrn}{\rrr^\notop}
% \newcommand{\sss}{\mathbf{s}}
% \newcommand{\ssn}{\sss^\notop}
% \newcommand{\uuu}{\mathbf{u}}
% \newcommand{\uun}{\mathbf{u}^\notop}
% \newcommand{\unn}{{u}^\notop}
% \newcommand{\vvv}{\mathbf{v}}
% \newcommand{\vvn}{\mathbf{v}^\notop}
% \newcommand{\vnn}{{v}^\notop}
% \newcommand{\www}{\mathbf{w}}
% \newcommand{\wwn}{\mathbf{w}^\notop}
% \newcommand{\wnn}{{w}^\notop}
% %
% % PHYSICS SYMBOLS
% \newcommand{\area}{\mathcal{A}}
% \newcommand{\aB}{{a^\notop_0}}
% \newcommand{\CCD}{C^{{}}_D}
% \newcommand{\cpm}{c^{{}}_\pm}
% \newcommand{\cpp}{c^{{}}_+}
% \newcommand{\cmm}{c^{{}}_-}
% \newcommand{\dktwopicubed}{\frac{d\kkk}{\twopicubed}}
% \newcommand{\Deln}{\Delta^\notop}
% \newcommand{\Ekin}{E^{{}}_\textrm{kin}}
% \newcommand{\ffe}{\fff^{{}}_\textrm{el}}
% \newcommand{\FFFdip}{\FFF^{{}}_\textrm{dip}}
% \newcommand{\FFFDEP}{\FFF^{{}}_\textrm{DEP}}
% \newcommand{\FFFdrag}{\FFF^{{}}_\textrm{drag}}
% \newcommand{\GC}{\mathcal{G}}
% \newcommand{\GCn}{\mathcal{G}^{{}}}
% \newcommand{\kB}{{k^\notop_\textrm{B}}}
% \newcommand{\kBT}{{k^\notop_\textrm{B} T}}
% \newcommand{\lcap}{\ell^{{}}_\textrm{cap}}
% \newcommand{\lcapsqr}{\ell^{2_{}}_\textrm{cap}}
% \newcommand{\len}{\mathcal{L}}
% \newcommand{\peo}{p^\notop_\textrm{eo}}
% \newcommand{\Qeo}{Q^\notop_\textrm{eo}}
% \newcommand{\QeoS}{Q^{*_{}}_\textrm{eo}}
% \newcommand{\Rh}{R^{{}}_\textrm{hyd}}
% \newcommand{\RhS}{R^{*_{}}_\textrm{hyd}}
% \newcommand{\Rhyd}{R^{{}}_\textrm{hyd}}
% \newcommand{\DPsurf}{\Delta p^{{}}_\textrm{surf}}
% \newcommand{\tcap}{\tau^{{}}_\textrm{cap}}
% \newcommand{\tadv}{\tau^{{}}_\textrm{adv}}
% \newcommand{\vol}{\mathcal{V}}
% \newcommand{\veo}{\vnn_\textrm{eo}}

% \newcommand{\deltan}{\delta^\notop}
% \newcommand{\eps}{\epsilon}
% \newcommand{\epsO}{\epsilon^\notop_0}
% %\newcommand{\epsI}{\epsilon^\notop_1}
% %\newcommand{\epsII}{\epsilon^\notop_2}
% %\newcommand{\epsr}{\epsilon^\notop_r}
% \newcommand{\bfGamma}{\mbox{$\Gamma$\hspace*{-0.6em}$\Gamma$}}
% \newcommand{\lamD}{\lambda^{{}}_D}
% \newcommand{\lamDsqr}{\lambda^{{2}}_D}
% \newcommand{\muO}{\mu^{{}}_0}
% \newcommand{\muion}{\mu^\notop_\textrm{ion}}
% \newcommand{\mueo}{\mu^\notop_\textrm{eo}}
% \newcommand{\oD}{{\omega^\notop_\textrm{D}}}
% \newcommand{\phin}{\phi^{{}}}
% \newcommand{\twopicubed}{(2\pi)^3}
% \newcommand{\rhoe}{\rho^\notop_\textrm{el}}
% \newcommand{\rhon}{\rho^\notop}
% \newcommand{\sigmae}{\sigma^\notop_\textrm{el}}
% \newcommand{\sigmaI}{\sigma^\notop_\textrm{el,1}}
% \newcommand{\sigmaII}{\sigma^\notop_\textrm{el,2}}
% \newcommand{\sigmaion}{\sigma^\notop_\textrm{ion}}
% \newcommand{\sigman}{\sigma^\notop}
% \newcommand{\domegatwopi}{\frac{d\omega}{2\pi}}
% %
% % Symbols with a tilde
% \newcommand{\Lti}{{\tilde{L}^{{}}{}}}
% \newcommand{\pti}{{\tilde{p}^{{}}{}}}
% \newcommand{\ppti}{{\tilde{\partial}^{{}}{}}}
% \newcommand{\rti}{{\tilde{r}^{{}}{}}}
% \newcommand{\rrrti}{{\tilde{\rrr}^{{}}{}}}
% \newcommand{\tti}{{\tilde{t}^{{}}{}}}
% \newcommand{\uti}{{\tilde{u}^{{}}{}}}
% \newcommand{\utin}{{\tilde{u}^{{}}_n{}}}
% \newcommand{\utim}{{\tilde{u}^{{}}_m{}}}
% \newcommand{\vti}{{\tilde{v}^{{}}{}}}
% \newcommand{\vxti}{{\tilde{v}^{{}}_x{}}}
% \newcommand{\vvvti}{{\tilde{\vvv}^{{}}{}}}
% \newcommand{\xti}{{\tilde{x}^{{}}{}}}
% \newcommand{\yti}{{\tilde{y}^{{}}{}}}
% \newcommand{\zti}{{\tilde{z}^{{}}{}}}
% \newcommand{\phiti}{{\tilde{\phi}^{{}}{}}}
% \newcommand{\nablati}{{\tilde{\nablabf}^{{}}{}}}
% \newcommand{\gamti}{\tilde{\gamma}}
% \newcommand{\omti}{\tilde{\omega}}
% %\newcommand{\Omti}{\tilde{\Omega}}
% \newcommand{\kti}{\tilde{k}}
% \newcommand{\komti}[1]{\tilde{k}_{\omega_0}^{(#1)}}
% \newcommand{\bti}{\tilde{b}}
% %
% % Symbols with a dot
% \newcommand{\Qdot}{\dot{Q}}
% \newcommand{\ydot}{\dot{y}}
% %
% % Symbols with a bar
% %\newcommand{\Qbar}{\bar{Q}}
% %\newcommand{\Gbar}{\bar{G}}
% \newcommand{\Abar}{\bar{A}}
% %
% % Symbols with a subscript 0
% \newcommand{\cO}{c^{{}}_0}
% \newcommand{\EO}{E^{{}}_0}
% \newcommand{\HO}{H^{{}}_0}
% \newcommand{\LO}{L^{{}}_0}
% \newcommand{\LOsqr}{L^{2_{}}_0}
% \newcommand{\NO}{N^{{}}_0}
% \newcommand{\pO}{p^{{}}_0}
% \newcommand{\PO}{P^{{}}_0}
% \newcommand{\rO}{r^{{}}_0}
% \newcommand{\TO}{T^{{}}_0}
% \newcommand{\VO}{V^{{}}_0}
% \newcommand{\vO}{v^{{}}_0}
% \newcommand{\phiO}{\phi^{{}}_0}
% %
% % Symbols with a superscript (0)
% \newcommand{\utiO}{\tilde{u}^{(0)_{}}}
% \newcommand{\util}{\tilde{u}^{(1)_{}}}
% \newcommand{\TTO}{T^{(0)_{}}}
% %
% % Symbols with a subscript ext, eq, eff
% \newcommand{\Deff}{D^{{}}_\textrm{eff}}
% \newcommand{\JJJeti}{\tilde{\JJJ}^{\textrm{el}_{}}}
% \newcommand{\cext}{c^{{}}_\textrm{ext}}
% \newcommand{\ceq}{c^{{}}_\textrm{eq}}
% \newcommand{\EEEext}{\EEn_\textrm{ext}}
% \newcommand{\pext}{p^{{}}_\textrm{ext}}
% \newcommand{\peq}{p^{{}}_\textrm{eq}}
% \newcommand{\phiext}{\phi^{{}}_\textrm{ext}}
% \newcommand{\phieq}{\phi^{{}}_\textrm{eq}}
% \newcommand{\phidip}{\phi^{{}}_\textrm{dip}}
% \newcommand{\phitot}{\phi^{{}}_\textrm{tot}}
% \newcommand{\rhoeext}{\rho^{\textrm{ext}_{}}_\textrm{el}}
% \newcommand{\rhoeeq}{\rho^{\textrm{eq}_{}}_\textrm{el}}
% %
% % SI units
% \newcommand{\SIC}{^\circ\textrm{C}}
% \newcommand{\SIF}{\textrm{F}}
% \newcommand{\SIHz}{\textrm{Hz}}
% \newcommand{\SIkHz}{\textrm{kHz}}
% \newcommand{\SIJ}{\textrm{J}}
% \newcommand{\SImJ}{\textrm{mJ}}
% \newcommand{\SIK}{\textrm{K}}
% \newcommand{\SIL}{\textrm{L}}
% \newcommand{\SImL}{\textrm{mL}}
% \newcommand{\SImuL}{\textrm{$\mu$L}}
% \newcommand{\SInL}{\textrm{nL}}
% \newcommand{\SIkg}{\textrm{kg}}
% \newcommand{\SIm}{\textrm{m}}
% \newcommand{\SImm}{\textrm{mm}}
% \newcommand{\SImum}{\textrm{$\mu$m}}
% \newcommand{\SInm}{\textrm{nm}}
% %\newcommand{\SIN}{\textrm{N}}
% \newcommand{\SIPa}{\textrm{Pa}}
% \newcommand{\SImPa}{\textrm{mPa}}
% \newcommand{\SIPas}{\textrm{Pa}\:\textrm{s}}
% \newcommand{\SImPas}{\textrm{mPa}\:\textrm{s}}
% \newcommand{\SIs}{\textrm{s}}
% \newcommand{\SIV}{\textrm{V}}
% \newcommand{\SIeV}{\textrm{eV}}
% \newcommand{\SImeV}{\textrm{meV}}
% %%
% %
% % DIRAC NOTATION
% \newcommand{\bra}[1]{\langle #1 |}
% \newcommand{\ket}[1]{|#1\rangle}
% \newcommand{\braket}[2]{\langle #1 | #2 \rangle}
% \newcommand{\bigbra}[1]{\big\langle #1 \big|}
% \newcommand{\bigket}[1]{\big| #1 \big\rangle}
% \newcommand{\bigbraket}[2]{\big\langle #1 \big| #2 \big\rangle}
% %
% % EQUATIONS

% % \newcommand{\beq}[1]{\begin{equation} \eqlab{#1}}
% % \newcommand{\eeq}{\end{equation}}
% %\newcommand{\bal}{\begin{align}}
% %\newcommand{\eal}{\end{align}}
% %\newcommand{\balnn}{\begin{align*}}
% %\newcommand{\ealnn}{\end{align*}}
% %\newcommand{\bsub}{\begin{subequations}}
% %\newcommand{\esub}{\end{subequations}}
% %\newcommand{\nn}{\nonumber}


